What do Toothbrushes do in the Kitchen? How Transformers Think our World is Structured

Transformer-based models are now predominant in NLP. They outperform approaches based on static models in many respects. This success has in turn prompted research that reveals a number of biases in the language models generated by transformers. In this paper we utilize this research on biases to investigate to what extent transformer-based language models allow for extracting knowledge about object relations (X occurs in Y; X consists of Z; action A involves using X). To this end, we compare contextualized models with their static counterparts. We make this comparison dependent on the application of a number of similarity measures and classifiers. Our results are threefold: Firstly, we show that the models combined with the different similarity measures differ greatly in terms of the amount of knowledge they allow for extracting. Secondly, our results suggest that similarity measures perform much worse than classifier-based approaches. Thirdly, we show that, surprisingly, static models perform almost as well as contextualized models -- in some cases even better.

==> tabellen/tab_obj_part.tex <==
\begin{table}[!hpt]
    \centering
    \scriptsize
    \begin{tabularx}{\linewidth}{l | l | r}
    \toprule
    Room & Object & $P(r|o)$  \\ \midrule
    
    \multirow{10}{*}{bed} 
    & leg & 100.00 \\
    & box spring & 100.00 \\
    & pillow & 100.00 \\
    & pillow protector & 100.00 \\
    & footboard & 100.00 \\
    & mattress cover & 100.00 \\
    & bolster & 100.00 \\
    & headboard & 100.00 \\
    & mattress & 100.00 \\
    & elastic & 100.00 \\ \midrule
    
    \multirow{19}{*}{refrigerator} 
    & freezer door & 100.00 \\
    & magnetic gasket & 100.00 \\
    & refrigerator compartment & 100.00 \\
    & door shelf & 100.00 \\
    & crisper & 100.00 \\
    & switch & 100.00 \\
    & dairy compartment & 100.00 \\
    & glass cover & 100.00 \\
    & butter compartment & 100.00 \\
    & ice cube tray & 100.00 \\
    & door stop & 100.00 \\
    & shelf & 100.00 \\
    & guard rail & 100.00 \\
    & freezer compartment & 100.00 \\
    & meat keeper & 100.00 \\
    & shelf channel & 100.00 \\
    & storage door & 100.00 \\
    & thermostat control & 100.00 \\
    & egg tray & 100.00 \\ \midrule
    
    \multirow{16}{*}{door} 
    & cornice & 100.00 \\
    & bottom rail & 100.00 \\
    & hanging stile & 100.00 \\
    & lock rail & 100.00 \\
    & panel & 100.00 \\
    & hinge & 100.00 \\
    & header & 100.00 \\
    & jamb & 100.00 \\
    & threshold & 100.00 \\
    & shutting stile & 100.00 \\
    & weatherboard & 100.00 \\
    & doorknob & 100.00 \\
    & lock & 100.00 \\
    & entablature & 100.00 \\
    & middle panel & 100.00 \\
    & top rail & 100.00 \\\midrule
    
    \multirow{12}{*}{mortise lock}
    & cotter pin & 100.00 \\
    & cylinder & 100.00 \\
    & strike plate & 100.00 \\
    & faceplate & 100.00 \\
    & keyway & 100.00 \\
    & stator & 100.00 \\
    & dead bolt & 100.00 \\
    & rotor & 100.00 \\
    & ring & 100.00 \\
    & spring & 100.00 \\
    & cylinder case & 100.00 \\
    & key & 100.00 \\ \midrule
    
    \multirow{20}{*}{toilet} 
    & waste pipe & 100.00 \\
    & ball-cock supply valve & 100.00 \\
    & seat & 100.00 \\
    & tank lid & 100.00 \\
    & shutoff valve & 100.00 \\
    & conical washer & 100.00 \\
    & valve seat shaft & 100.00 \\
    & float ball & 100.00 \\
    & trip lever & 100.00 \\
    & refill tube & 100.00 \\
    & lift chain & 100.00 \\
    & toilet bowl & 100.00 \\
    & flush handle & 100.00 \\
    & wax seal & 100.00 \\
    & seat cover & 100.00 \\
    & cold-water supply line & 100.00 \\
    & filler tube & 100.00 \\
    & tank ball & 100.00 \\
    & overflow tube & 100.00 \\
    & trap & 100.00 \\ \bottomrule
    
    \end{tabularx}
    \caption{}
    \label{tab:obj-part}
\end{table}

==> tabellen/tab_room_obj.tex <==
\begin{table}[!hpt]
    \centering
    \scriptsize
    \begin{tabularx}{\linewidth}{l | l | r}
    \toprule
    Room & Object & $P(r|o)$  \\ \midrule
    
    \multirow{10}{*}{bathroom} 
    & toilet & 100.00 \\
    & bathtub & 100.00 \\
    & toothbrush holder & 100.00 \\
    & toothpaste & 100.00 \\
    & shower curtain & 100.00 \\
    & toothbrush & 96.93 \\
    & towel rod & 96.47 \\
    & toilet paper & 96.20 \\
    & squeeze tube & 95.00 \\
    & faucet handle & 82.30 \\ \midrule
    
    \multirow{10}{*}{bedroom} 
    & dresser & 100.00 \\
    & night stand & 100.00 \\ 
    & headboard & 100.00 \\
    & bed & 97.38 \\
    & alarm clock & 97.15 \\
    & laundry basket & 85.72 \\
    & hat & 74.13 \\
    & doll & 70.17 \\
    & stuffed animal & 59.90 \\
    & pillow & 55.64 \\ \midrule
    
    \multirow{10}{*}{kitchen} 
    & drying rack & 100.00 \\
    & kitchen island & 100.00 \\
    & pot & 100.00 \\
    & frying pan & 100.00 \\
    & spice rack & 100.00 \\
    & cutting board & 100.00 \\
    & blender & 100.00 \\
    & knife & 100.00 \\
    & stove & 97.66 \\
    & dishwasher & 97.21 \\\midrule
    
    \multirow{10}{*}{living room}
    & coffee table & 93.68 \\
    & ottoman & 93.00 \\
    & fireplace & 86.57 \\
    & dvd player & 69.39 \\
    & sofa & 68.33 \\
    & decorative plate & 60.59 \\
    & tv stand & 56.94 \\
    & blanket & 54.70 \\
    & television & 52.71 \\
    & remote control & 50.08 \\ \midrule
    
    \multirow{10}{*}{office} 
    & whiteboard & 100.00 \\
    & room divider & 93.87 \\
    & stapler & 92.21 \\
    & cork board & 91.80 \\
    & file & 87.77 \\
    & keyboard & 85.09 \\
    & mouse & 84.16 \\
    & pen & 83.35 \\
    & computer & 81.87 \\
    & column & 80.54 \\ \bottomrule
    
    \end{tabularx}
    \caption{Statistics generated from ScanNet using Nyu categories. The probability stands for the probability that it is exactly this space, under the condition that this object is given.}
    \label{tab:room-obj}
\end{table}

==> tabellen/tab_score_summary.tex <==
\begin{table*}
    \setlength{\tabcolsep}{3pt}
    \centering
    \scriptsize
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X }
    \toprule
    &  & \multicolumn{6}{c}{\textbf{Word2Vec}} & \multicolumn{6}{c}{\textbf{Glove}} & \multicolumn{6}{c}{\textbf{Levy}} & \multicolumn{6}{c}{\textbf{fastText}} \\ 
    &  & Cos & Dist & Pear & Spear & Kend & Clas & Cos & Dist & Pear & Spear & Kend & Clas & Cos & Dist & Pear & Spear & Kend & Clas & Cos & Dist & Pear & Spear & Kend & Clas \\ \midrule
    
    \multirow{5}{*}{\textbf{Room}} 
    & Bathroom & 0.34 & 0.37 & 0.37 & 0.37 & 0.37 & 0.69 & 0.35 & 0.38 & 0.37 & 0.37 & 0.37 & 0.97 & 0.33 & 0.38 & 0.36 & 0.37 & 0.37 & 0.53 & 0.45 & 0.51 & 0.50 & 0.50 & 0.50 & 0.91 \\
    
    & Bedroom & 0.21 & 0.21 & 0.21 & 0.21 & 0.21 & 0.63 & 0.31 & 0.29 & 0.31 & 0.31 & 0.31 & 0.60 & 0.18 & 0.20 & 0.20 & 0.20 & 0.20 & 0.15 & 0.29 & 0.31 & 0.29 & 0.31 & 0.31 & 0.74 \\

    & Kitchen & 0.37 & 0.36 & 0.36 & 0.36 & 0.36 & 0.65 & 0.40 & 0.42 & 0.39 & 0.43 & 0.43 & 0.83 & 0.15 & 0.17 & 0.16 & 0.16 & 0.17 & 0.46 & 0.33 & 0.35 & 0.38 & 0.34 & 0.34 & 0.82 \\
    
    & Living room & 0.36 & 0.22 & 0.23 & 0.21 & 0.21 & 0.38 & 0.27 & 0.27 & 0.30 & 0.26 & 0.26 & 0.62 & 0.16 & 0.23 & 0.22 & 0.23 & 0.23 & 0.42 & 0.18 & 0.26 & 0.26 & 0.28 & 0.27 & 0.69 \\
    
    & Office & 0.24 & 0.22 & 0.21 & 0.21 & 0.21 & 0.66 & 0.17 & 0.35 & 0.18 & 0.38 & 0.37 & 0.79 & 0.26 & 0.27 & 0.26 & 0.27 & 0.28 & 0.56 & 0.34 & 0.34 & 0.29 & 0.36 & 0.36 & 0.75 \\ \hline
    
    \rowstyle{\bfseries} & All & 0.24 & 0.23 & 0.23 & 0.23 & 0.23 & 0.61 & 0.26 & 0.32 & 0.28 & 0.33 & 0.33 & 0.77 & 0.14 & 0.15 & 0.16 & 0.14 & 0.15 & 0.39 & 0.26 & 0.31 & 0.31 & 0.31 & 0.31 & 0.78 \\ \midrule
    
    \multirow{6}{*}{\textbf{Part}} 
    & Bed & 0.42 & 0.43 & 0.42 & 0.40 & 0.41 & 0.56 & 0.41 & 0.50 & 0.36 & 0.48 & 0.48 & 0.81 & - & - & - & - & - & - & 0.52 & 0.53 & 0.46 & 0.52 & 0.53 & 0.66 \\
    
    & Dishwasher & 0.20 & 0.24 & 0.21 & 0.24 & 0.24 & 0.26 & 0.32 & 0.31 & 0.33 & 0.30 & 0.30 & 0.44 & - & - & - & - & - & - & 0.36 & 0.31 & 0.35 & 0.31 & 0.31 & 0.33 \\
    
    & Door & 0.12 & 0.11 & 0.12 & 0.12 & 0.12 & 0.78 & 0.17 & 0.21 & 0.14 & 0.22 & 0.22 & 0.79 & - & - & - & - & - & - & 0.21 & 0.25 & 0.24 & 0.22 & 0.23 & 0.86 \\
    
    & Mortise lock & 0.13 & 0.18 & 0.20 & 0.20 & 0.20 & 0.54 & 0.11 & 0.28 & 0.24 & 0.29 & 0.29 & 0.59 & - & - & - & - & - & - & 0.12 & 0.17 & 0.14 & 0.19 & 0.19 & 0.68 \\

    & Refrigerator & 0.36 & 0.42 & 0.41 & 0.40 & 0.41 & 0.66 & 0.52 & 0.56 & 0.54 & 0.55 & 0.55 & 0.72 & - & - & - & - & - & - & 0.51 & 0.58 & 0.54 & 0.59 & 0.58 & 0.78 \\

    & Toilet & 0.22 & 0.26 & 0.26 & 0.26 & 0.26 & 0.66 & 0.26 & 0.32 & 0.31 & 0.30 & 0.30 & 0.77 & - & - & - & - & - & - & 0.32 & 0.35 & 0.36 & 0.33 & 0.34 & 0.76 \\ \hline

    \rowstyle{\bfseries} & All & 0.16 & 0.27 & 0.26 & 0.26 & 0.26 & 0.58 & 0.23 & 0.34 & 0.29 & 0.34 & 0.34 & 0.68 & - & - & - & - & - & - & 0.24 & 0.34 & 0.30 & 0.34 & 0.34 & 0.69 \\ \midrule
    
    \multirow{6}{*}{\textbf{Verb}} 
    & eat & 0.79 & 0.79 & 0.78 & 0.76 & 0.77 & 0.91 & 0.77 & 0.86 & 0.77 & 0.79 & 0.80 & 0.92 & 0.45 & 0.44 & 0.45 & 0.45 & 0.45 & 0.86 & 0.75 & 0.80 & 0.74 & 0.79 & 0.79 & 0.87 \\
    
    & listen to & 0.56 & 0.66 & 0.55 & 0.58 & 0.58 & 0.48 & 0.49 & 0.71 & 0.56 & 0.65 & 0.66 & 0.59 & 0.31 & 0.30 & 0.32 & 0.31 & 0.30 & 0.48 & 0.34 & 0.47 & 0.39 & 0.54 & 0.54 & 0.50 \\

    & play & 0.65 & 0.70 & 0.64 & 0.64 & 0.64 & 0.66 & 0.65 & 0.80 & 0.65 & 0.71 & 0.72 & 0.56 & 0.45 & 0.45 & 0.44 & 0.44 & 0.44 & 0.58 & 0.64 & 0.70 & 0.64 & 0.69 & 0.69 & 0.55 \\
    
    & read & 0.42 & 0.52 & 0.43 & 0.47 & 0.48 & 0.69 & 0.50 & 0.60 & 0.52 & 0.58 & 0.58 & 0.64 & 0.34 & 0.32 & 0.33 & 0.31 & 0.32 & 0.54 & 0.53 & 0.56 & 0.54 & 0.59 & 0.59 & 0.62 \\
    
    & wash with & 0.42 & 0.52 & 0.52 & 0.51 & 0.51 & 0.63 & 0.45 & 0.57 & 0.49 & 0.52 & 0.52 & 0.66 & 0.35 & 0.32 & 0.35 & 0.33 & 0.33 & 0.63 & 0.33 & 0.52 & 0.45 & 0.50 & 0.51 & 0.70 \\
    
    & wear & 0.76 & 0.78 & 0.76 & 0.75 & 0.76 & 0.85 & 0.81 & 0.87 & 0.81 & 0.84 & 0.84 & 0.86 & 0.59 & 0.55 & 0.58 & 0.52 & 0.52 & 0.80 & 0.79 & 0.81 & 0.78 & 0.79 & 0.79 & 0.85 \\ \hline
    
    \rowstyle{\bfseries} & All & 0.55 & 0.60 & 0.57 & 0.57 & 0.57 & 0.70 & 0.58 & 0.68 & 0.60 & 0.64 & 0.64 & 0.72 & 0.35 & 0.33 & 0.35 & 0.33 & 0.33 & 0.66 & 0.48 & 0.58 & 0.51 & 0.57 & 0.57 & 0.69 \\
    
    %Social &  & & - &  & & - &  & & - &  & & - & \\ 
    \bottomrule
    \end{tabularx}
    \caption{Static Summary}
    \label{tab:static-score-summary}
\end{table*}


\begin{table*}
    \centering
    \setlength{\tabcolsep}{3pt}
    \scriptsize
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X | ^X ^X ^X ^X | ^X ^X ^X ^X | ^X ^X ^X ^X | ^X ^X ^X ^X}
    \toprule
    &  & \multicolumn{4}{c}{\textbf{BERT-Base}} & \multicolumn{4}{c}{\textbf{BERT-Large}} & \multicolumn{4}{c}{\textbf{RoBERTa}} & \multicolumn{4}{c}{\textbf{ELECTRA}} & \multicolumn{4}{c}{\textbf{ALBERT }} \\ 
    &  & Cos & Dist & Log & Clas & Cos & Dist & Log & Clas & Cos & Dist & Log & Clas & Cos & Dist & Log & Clas & Cos & Dist & Log & Clas \\ \midrule
    
    \multirow{5}{*}{\textbf{Room}} 
    & Bathroom & 0.58 & 0.14 & 0.52 & 0.91 & 0.65 & 0.14 & 0.59 & 0.99 & 0.22 & 0.18 & 0.43 & 0.99 & 0.58 & 0.17 & 0.34 & 0.84 & 0.25 & 0.15 & 0.39 & 0.94 \\
    & Bedroom & 0.48 & 0.31 & 0.43 & 0.74 & 0.45 & 0.24 & 0.44 & 0.78 & 0.22 & 0.21 & 0.22 & 0.62 & 0.31 & 0.16 & 0.37 & 0.48 & 0.22 & 0.24 & 0.47 & 0.83 \\
    & Kitchen & 0.57 & 0.15 & 0.58 & 0.75 & 0.43 & 0.18 & 0.54 & 0.77 & 0.39 & 0.25 & 0.17 & 0.81 & 0.34 & 0.17 & 0.36 & 0.65 & 0.26 & 0.13 & 0.30 & 0.71 \\
    & Living room & 0.31 & 0.15 & 0.26 & 0.69 & 0.23 & 0.21 & 0.24 & 0.56 & 0.15 & 0.18 & 0.20 & 0.77 & 0.26 & 0.14 & 0.33 & 0.43 & 0.15 & 0.13 & 0.54 & 0.67 \\
    & Office & 0.47 & 0.19 & 0.28 & 0.62 & 0.41 & 0.19 & 0.31 & 0.68 & 0.15 & 0.14 & 0.53 & 0.74 & 0.16 & 0.17 & 0.23 & 0.47 & 0.23 & 0.18 & 0.42 & 0.86 \\ \hline
    \rowstyle{\bfseries}& All & 0.43 & 0.08 & 0.33 & 0.74 & 0.34 & 0.08 & 0.36 & 0.77 & 0.19 & 0.09 & 0.27 & 0.79 & 0.22 & 0.08 & 0.27 & 0.57 & 0.19 & 0.06 & 0.23 & 0.80 \\ \midrule
   
    \multirow{6}{*}{\textbf{Part}} 
    & Bed & 0.55 & 0.12 & 0.51 & 0.70 & 0.49 & 0.25 & 0.55 & 0.70 & 0.20 & 0.10 & 0.62 & 0.53 & 0.37 & 0.10 & 0.43 & 0.63 & 0.26 & 0.11 & 0.54 & 0.65 \\
    
    & Dishwasher & 0.22 & 0.11 & 0.22 & 0.37 & 0.30 & 0.12 & 0.31 & 0.26 & 0.16 & 0.22 & 0.19 & 0.23 & 0.26 & 0.12 & 0.21 & 0.36 & 0.17 & 0.10 & 0.25 & 0.26 \\
    
    & Door & 0.19 & 0.26 & 0.20 & 0.68 & 0.13 & 0.12 & 0.39 & 0.64 & 0.15 & 0.18 & 0.27 & 0.53 & 0.14 & 0.23 & 0.17 & 0.63 & 0.13 & 0.11 & 0.21 & 0.57 \\
    
    & Mortise lock & 0.12 & 0.13 & 0.09 & 0.35 & 0.14 & 0.17 & 0.11 & 0.46 & 0.07 & 0.16 & 0.12 & 0.35 & 0.16 & 0.17 & 0.15 & 0.47 & 0.09 & 0.34 & 0.22 & 0.53 \\
    
    & Refrigerator & 0.44 & 0.18 & 0.40 & 0.66 & 0.38 & 0.17 & 0.54 & 0.58 & 0.18 & 0.30 & 0.45 & 0.62 & 0.37 & 0.19 & 0.43 & 0.53 & 0.44 & 0.21 & 0.51 & 0.70 \\
    
    & Toilet & 0.18 & 0.18 & 0.29 & 0.37 & 0.25 & 0.12 & 0.26 & 0.49 & 0.22 & 0.18 & 0.41 & 0.47 & 0.34 & 0.12 & 0.42 & 0.56 & 0.24 & 0.11 & 0.25 & 0.51 \\ \hline
    
    \rowstyle{\bfseries} & All & 0.20 & 0.07 & 0.24 & 0.52 & 0.22 & 0.06 & 0.28 & 0.51 & 0.07 & 0.08 & 0.29 & 0.46 & 0.21 & 0.04 & 0.23 & 0.53 & 0.08 & 0.03 & 0.27 & 0.53 \\ \midrule
    
    
    \multirow{6}{*}{\textbf{Verb}} 
    & eat & 0.78 & 0.20 & 0.67 & 0.87 & 0.65 & 0.19 & 0.72 & 0.84 & 0.26 & 0.19 & 0.81 & 0.80 & 0.62 & 0.19 & 0.76 & 0.79 & 0.53 & 0.18 & 0.74 & 0.85 \\
    
    & listen to & 0.46 & 0.18 & 0.51 & 0.62 & 0.50 & 0.56 & 0.50 & 0.60 & 0.30 & 0.22 & 0.55 & 0.51 & 0.57 & 0.27 & 0.59 & 0.46 & 0.23 & 0.36 & 0.51 & 0.63 \\
    
    & play & 0.63 & 0.31 & 0.69 & 0.70 & 0.55 & 0.23 & 0.73 & 0.66 & 0.37 & 0.14 & 0.65 & 0.55 & 0.64 & 0.25 & 0.69 & 0.68 & 0.37 & 0.23 & 0.52 & 0.63 \\
    
    & read & 0.42 & 0.19 & 0.65 & 0.73 & 0.30 & 0.21 & 0.66 & 0.78 & 0.26 & 0.32 & 0.59 & 0.57 & 0.41 & 0.25 & 0.63 & 0.68 & 0.31 & 0.36 & 0.57 & 0.64 \\
    
    & wash with & 0.49 & 0.34 & 0.33 & 0.65 & 0.42 & 0.43 & 0.45 & 0.63 & 0.30 & 0.20 & 0.30 & 0.64 & 0.42 & 0.17 & 0.35 & 0.57 & 0.33 & 0.17 & 0.32 & 0.62 \\
    
    & wear & 0.66 & 0.15 & 0.76 & 0.92 & 0.62 & 0.20 & 0.74 & 0.93 & 0.24 & 0.12 & 0.77 & 0.70 & 0.53 & 0.13 & 0.74 & 0.87 & 0.30 & 0.19 & 0.77 & 0.85 \\ \hline

    \rowstyle{\bfseries} & All & 0.53 & 0.11 & 0.38 & 0.74 & 0.37 & 0.16 & 0.44 & 0.74 & 0.20 & 0.09 & 0.37 & 0.62 & 0.49 & 0.07 & 0.37 & 0.67 & 0.15 & 0.09 & 0.26 & 0.70 \\
    %Verb &  & & &  & & &  & & &  & & & \\ \midrule
    
    %Social &  & & &  & & &  & & &  & & & \\ 
    \bottomrule
    \end{tabularx}
    \caption{Masked Summary}
    \label{tab:masked-score-summary}
\end{table*}


\begin{table*}
    \centering
    \setlength{\tabcolsep}{3pt}
    \scriptsize
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X ^X }
    \toprule
    &  & \multicolumn{7}{c}{\textbf{GPT2}} & \multicolumn{7}{c}{\textbf{GPT-Neo}} & \multicolumn{7}{c}{\textbf{GPT-J}} \\ 
    &  & Cos & Dist & Obj & ObjL & R & RL & Clas & Cos & Dist & Obj & ObjL & R & RL & Clas & Cos & Dist & Obj & ObjL & R & RL & Clas \\ \midrule
    
    \multirow{5}{*}{\textbf{Room}} 
    & Bathroom & 0.51 & 0.39 & 0.30 & 0.53 & 0.50 & 0.37 & 0.96 & 0.28 & 0.32 & 0.54 & 0.62 & 0.36 & 0.25 & 0.99 & 0.50 & 0.24 & 0.68 & 0.66 & 0.66 & 0.48 & 0.94 \\
    & Bedroom & 0.26 & 0.13 & 0.26 & 0.37 & 0.47 & 0.38 & 0.56 & 0.19 & 0.21 & 0.53 & 0.45 & 0.53 & 0.48 & 0.72 & 0.24 & 0.22 & 0.49 & 0.40 & 0.62 & 0.48 & 0.70 \\
    & Kitchen & 0.33 & 0.15 & 0.28 & 0.54 & 0.69 & 0.60 & 0.85 & 0.30 & 0.16 & 0.46 & 0.73 & 0.70 & 0.57 & 0.88 & 0.33 & 0.17 & 0.27 & 0.64 & 0.83 & 0.70 & 0.81 \\
    & Living room & 0.22 & 0.21 & 0.40 & 0.43 & 0.41 & 0.33 & 0.42 & 0.27 & 0.25 & 0.62 & 0.65 & 0.60 & 0.44 & 0.63 & 0.22 & 0.22 & 0.60 & 0.66 & 0.67 & 0.45 & 0.64 \\
    & Office & 0.13 & 0.26 & 0.47 & 0.36 & 0.37 & 0.23 & 0.85 & 0.32 & 0.16 & 0.52 & 0.38 & 0.46 & 0.34 & 0.89 & 0.23 & 0.42 & 0.54 & 0.50 & 0.49 & 0.39 & 0.80 \\ \hline
    \rowstyle{\bfseries}& All & 0.26 & 0.08 & 0.27 & 0.43 & 0.46 & 0.33 & 0.74 & 0.15 & 0.09 & 0.48 & 0.56 & 0.44 & 0.36 & 0.83 & 0.23 & 0.08 & 0.48 & 0.56 & 0.56 & 0.38 & 0.78 \\ \midrule
   
   
    \multirow{6}{*}{\textbf{Part}} 
    & Bed & 0.36 & 0.07 & 0.52 & 0.68 & 0.67 & 0.45 & 0.63 & 0.32 & 0.11 & 0.61 & 0.65 & 0.77 & 0.70 & 0.80 & 0.46 & 0.09 & 0.63 & 0.68 & 0.81 & 0.68 & 0.73 \\
    
    & Dishwasher & 0.11 & 0.08 & 0.34 & 0.43 & 0.25 & 0.23 & 0.33 & 0.06 & 0.12 & 0.45 & 0.50 & 0.30 & 0.29 & 0.25 & 0.09 & 0.13 & 0.49 & 0.51 & 0.44 & 0.38 & 0.35 \\
    
    & Door & 0.23 & 0.09 & 0.12 & 0.24 & 0.20 & 0.28 & 0.58 & 0.27 & 0.24 & 0.23 & 0.27 & 0.35 & 0.42 & 0.66 & 0.15 & 0.17 & 0.34 & 0.37 & 0.37 & 0.41 & 0.72 \\
    
    & Mortise lock & 0.07 & 0.10 & 0.39 & 0.44 & 0.17 & 0.18 & 0.54 & 0.11 & 0.19 & 0.46 & 0.52 & 0.30 & 0.22 & 0.60 & 0.15 & 0.33 & 0.52 & 0.51 & 0.47 & 0.31 & 0.57 \\
    
    & Refrigerator & 0.42 & 0.20 & 0.57 & 0.30 & 0.53 & 0.52 & 0.64 & 0.29 & 0.30 & 0.44 & 0.40 & 0.47 & 0.55 & 0.64 & 0.46 & 0.11 & 0.45 & 0.42 & 0.57 & 0.63 & 0.62 \\
    
    & Toilet & 0.29 & 0.08 & 0.31 & 0.42 & 0.20 & 0.17 & 0.57 & 0.27 & 0.17 & 0.50 & 0.57 & 0.25 & 0.26 & 0.52 & 0.32 & 0.13 & 0.45 & 0.55 & 0.32 & 0.37 & 0.59 \\\hline
    
    \rowstyle{\bfseries}& All & 0.14 & 0.04 & 0.34 & 0.39 & 0.28 & 0.25 & 0.55 & 0.12 & 0.09 & 0.44 & 0.47 & 0.37 & 0.36 & 0.57 & 0.16 & 0.05 & 0.47 & 0.49 & 0.42 & 0.43 & 0.59 \\ \midrule
    
    \multirow{6}{*}{\textbf{Verb}} 
    & eat & 0.49 & 0.82 & 0.65 & - & - & 0.84 & 0.45 & 0.86 & 0.66 & - & - & 0.86 & 0.48 & 0.68 & 0.74 & - & - & 0.90 \\
    
    & listen to & 0.22 & 0.57 & 0.51 & - & - & 0.57 & 0.22 & 0.47 & 0.47 & - & - & 0.49 & 0.21 & 0.60 & 0.56 & - & - & 0.57 \\
    
    & play & 0.40 & 0.64 & 0.62 & - & - & 0.61 & 0.32 & 0.66 & 0.61 & - & - & 0.59 & 0.34 & 0.66 & 0.70 & - & - & 0.68 \\
    
    & read & 0.32 & 0.63 & 0.30 & - & - & 0.51 & 0.32 & 0.61 & 0.34 & - & - & 0.46 & 0.40 & 0.63 & 0.41 & - & - & 0.60 \\
    
    & wash with & 0.39 & 0.77 & 0.51 & - & - & 0.57 & 0.28 & 0.66 & 0.52 & - & - & 0.57 & 0.23 & 0.69 & 0.52 & - & - & 0.65 \\
    
    & wear & 0.44 & 0.38 & 0.72 & - & - & 0.85 & 0.16 & 0.39 & 0.66 & - & - & 0.83 & 0.21 & 0.38 & 0.62 & - & - & 0.87 \\ \midrule
    
    \rowstyle{\bfseries}& All & 0.31 & 0.52 & 0.53 & - & - & 0.66 & 0.19 & 0.49 & 0.52 & - & - & 0.63 & 0.23 & 0.50 & 0.56 & - & - & 0.71 \\ \bottomrule

    \end{tabularx}
    \caption{GPT Summary}
    \label{tab:gpt-score-summary}
\end{table*}

==> tabellen/tab_score_summary_v2.tex <==
\begin{table*}
    \setlength{\tabcolsep}{2pt}
    \centering
    \scriptsize
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X }
    \toprule
    &  & \multicolumn{6}{c}{\textbf{Word2Vec}} & \multicolumn{6}{c}{\textbf{Glove}} & \multicolumn{6}{c}{\textbf{Levy}} & \multicolumn{6}{c}{\textbf{fastText}} \\ 
    &  & Cos & Dist & Pear & Spear & Kend & Clas & Cos & Dist & Pear & Spear & Kend & Clas & Cos & Dist & Pear & Spear & Kend & Clas & Cos & Dist & Pear & Spear & Kend & Clas \\ \midrule
    
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}} 
    & Bathroom & 0.34 & 0.37 & 0.37 & 0.37 & 0.37 & 0.69 & 0.35 & 0.38 & 0.37 & 0.37 & 0.37 & 0.97 & 0.33 & 0.38 & 0.36 & 0.37 & 0.37 & 0.53 & 0.45 & 0.51 & 0.50 & 0.50 & 0.50 & 0.91 \\
    
    & Bedroom & 0.21 & 0.21 & 0.21 & 0.21 & 0.21 & 0.63 & 0.31 & 0.29 & 0.31 & 0.31 & 0.31 & 0.60 & 0.18 & 0.20 & 0.20 & 0.20 & 0.20 & 0.15 & 0.29 & 0.31 & 0.29 & 0.31 & 0.31 & 0.74 \\

    & Kitchen & 0.37 & 0.36 & 0.36 & 0.36 & 0.36 & 0.65 & 0.40 & 0.42 & 0.39 & 0.43 & 0.43 & 0.83 & 0.15 & 0.17 & 0.16 & 0.16 & 0.17 & 0.46 & 0.33 & 0.35 & 0.38 & 0.34 & 0.34 & 0.82 \\
    
    & Living room & 0.36 & 0.22 & 0.23 & 0.21 & 0.21 & 0.38 & 0.27 & 0.27 & 0.30 & 0.26 & 0.26 & 0.62 & 0.16 & 0.23 & 0.22 & 0.23 & 0.23 & 0.42 & 0.18 & 0.26 & 0.26 & 0.28 & 0.27 & 0.69 \\
    
    & Office & 0.24 & 0.22 & 0.21 & 0.21 & 0.21 & 0.66 & 0.17 & 0.35 & 0.18 & 0.38 & 0.37 & 0.79 & 0.26 & 0.27 & 0.26 & 0.27 & 0.28 & 0.56 & 0.34 & 0.34 & 0.29 & 0.36 & 0.36 & 0.75 \\ \hline
    
    \rowstyle{\bfseries} & All & 0.24 & 0.23 & 0.23 & 0.23 & 0.23 & 0.61 & 0.26 & 0.32 & 0.28 & 0.33 & 0.33 & 0.77 & 0.14 & 0.15 & 0.16 & 0.14 & 0.15 & 0.39 & 0.26 & 0.31 & 0.31 & 0.31 & 0.31 & 0.78 \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}} 
    & Bed & 0.42 & 0.43 & 0.42 & 0.40 & 0.41 & 0.56 & 0.41 & 0.50 & 0.36 & 0.48 & 0.48 & 0.81 & - & - & - & - & - & - & 0.52 & 0.53 & 0.46 & 0.52 & 0.53 & 0.66 \\
    
    & Dishwasher & 0.20 & 0.24 & 0.21 & 0.24 & 0.24 & 0.26 & 0.32 & 0.31 & 0.33 & 0.30 & 0.30 & 0.44 & - & - & - & - & - & - & 0.36 & 0.31 & 0.35 & 0.31 & 0.31 & 0.33 \\
    
    & Door & 0.12 & 0.11 & 0.12 & 0.12 & 0.12 & 0.78 & 0.17 & 0.21 & 0.14 & 0.22 & 0.22 & 0.79 & - & - & - & - & - & - & 0.21 & 0.25 & 0.24 & 0.22 & 0.23 & 0.86 \\
    
    & Mortise lock & 0.13 & 0.18 & 0.20 & 0.20 & 0.20 & 0.54 & 0.11 & 0.28 & 0.24 & 0.29 & 0.29 & 0.59 & - & - & - & - & - & - & 0.12 & 0.17 & 0.14 & 0.19 & 0.19 & 0.68 \\

    & Refrigerator & 0.36 & 0.42 & 0.41 & 0.40 & 0.41 & 0.66 & 0.52 & 0.56 & 0.54 & 0.55 & 0.55 & 0.72 & - & - & - & - & - & - & 0.51 & 0.58 & 0.54 & 0.59 & 0.58 & 0.78 \\

    & Toilet & 0.22 & 0.26 & 0.26 & 0.26 & 0.26 & 0.66 & 0.26 & 0.32 & 0.31 & 0.30 & 0.30 & 0.77 & - & - & - & - & - & - & 0.32 & 0.35 & 0.36 & 0.33 & 0.34 & 0.76 \\ \hline

    \rowstyle{\bfseries} & All & 0.16 & 0.27 & 0.26 & 0.26 & 0.26 & 0.58 & 0.23 & 0.34 & 0.29 & 0.34 & 0.34 & 0.68 & - & - & - & - & - & - & 0.24 & 0.34 & 0.30 & 0.34 & 0.34 & 0.69 \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}}
    & eat & 0.79 & 0.79 & 0.78 & 0.76 & 0.77 & 0.91 & 0.77 & 0.86 & 0.77 & 0.79 & 0.80 & 0.92 & 0.45 & 0.44 & 0.45 & 0.45 & 0.45 & 0.86 & 0.75 & 0.80 & 0.74 & 0.79 & 0.79 & 0.87 \\
    
    & listen to & 0.56 & 0.66 & 0.55 & 0.58 & 0.58 & 0.48 & 0.49 & 0.71 & 0.56 & 0.65 & 0.66 & 0.59 & 0.31 & 0.30 & 0.32 & 0.31 & 0.30 & 0.48 & 0.34 & 0.47 & 0.39 & 0.54 & 0.54 & 0.50 \\

    & play & 0.65 & 0.70 & 0.64 & 0.64 & 0.64 & 0.66 & 0.65 & 0.80 & 0.65 & 0.71 & 0.72 & 0.56 & 0.45 & 0.45 & 0.44 & 0.44 & 0.44 & 0.58 & 0.64 & 0.70 & 0.64 & 0.69 & 0.69 & 0.55 \\
    
    & read & 0.42 & 0.52 & 0.43 & 0.47 & 0.48 & 0.69 & 0.50 & 0.60 & 0.52 & 0.58 & 0.58 & 0.64 & 0.34 & 0.32 & 0.33 & 0.31 & 0.32 & 0.54 & 0.53 & 0.56 & 0.54 & 0.59 & 0.59 & 0.62 \\
    
    & wash with & 0.42 & 0.52 & 0.52 & 0.51 & 0.51 & 0.63 & 0.45 & 0.57 & 0.49 & 0.52 & 0.52 & 0.66 & 0.35 & 0.32 & 0.35 & 0.33 & 0.33 & 0.63 & 0.33 & 0.52 & 0.45 & 0.50 & 0.51 & 0.70 \\
    
    & wear & 0.76 & 0.78 & 0.76 & 0.75 & 0.76 & 0.85 & 0.81 & 0.87 & 0.81 & 0.84 & 0.84 & 0.86 & 0.59 & 0.55 & 0.58 & 0.52 & 0.52 & 0.80 & 0.79 & 0.81 & 0.78 & 0.79 & 0.79 & 0.85 \\ \hline
    
    \rowstyle{\bfseries} & All & 0.55 & 0.60 & 0.57 & 0.57 & 0.57 & 0.70 & 0.58 & 0.68 & 0.60 & 0.64 & 0.64 & 0.72 & 0.35 & 0.33 & 0.35 & 0.33 & 0.33 & 0.66 & 0.48 & 0.58 & 0.51 & 0.57 & 0.57 & 0.69 \\
    
    %Social &  & & - &  & & - &  & & - &  & & - & \\ 
    \bottomrule
    \end{tabularx}
    \caption{All results of the static models.}
    \label{tab:static-score-summary}
\end{table*}


\begin{table*}
    \centering
    \setlength{\tabcolsep}{2pt}
    \scriptsize
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X | ^X ^X ^X ^X | ^X ^X ^X ^X | ^X ^X ^X ^X | ^X ^X ^X ^X}
    \toprule
    &  & \multicolumn{4}{c}{\textbf{BERT-Base}} & \multicolumn{4}{c}{\textbf{BERT-Large}} & \multicolumn{4}{c}{\textbf{RoBERTa}} & \multicolumn{4}{c}{\textbf{ElectraGen}} & \multicolumn{4}{c}{\textbf{Albert}} \\ 
    &  & Cos & M-I & M-C & Clas & Cos & M-I & M-C & Clas & Cos & M-I & M-C & Clas & Cos & M-I & M-C & Clas & Cos & M-C & M-I & Clas \\ \midrule
    
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}} 
    & Bathroom & 0.57 & 0.13 & 0.52 & 0.92 & 0.65 & 0.30 & 0.59 & 0.99 & 0.21 & 0.24 & 0.52 & 0.98 & 0.58 & 0.32 & 0.34 & 0.86 & 0.24 & 0.18 & 0.39 & 0.94 \\
    & Bedroom & 0.48 & 0.33 & 0.43 & 0.74 & 0.44 & 0.41 & 0.44 & 0.80 & 0.23 & 0.18 & 0.36 & 0.59 & 0.32 & 0.31 & 0.37 & 0.51 & 0.23 & 0.22 & 0.47 & 0.84 \\
    & Kitchen & 0.56 & 0.25 & 0.58 & 0.75 & 0.43 & 0.24 & 0.54 & 0.76 & 0.39 & 0.27 & 0.59 & 0.82 & 0.34 & 0.24 & 0.36 & 0.65 & 0.25 & 0.17 & 0.30 & 0.68 \\
    & Living room & 0.30 & 0.37 & 0.26 & 0.68 & 0.23 & 0.38 & 0.24 & 0.57 & 0.13 & 0.38 & 0.28 & 0.77 & 0.26 & 0.48 & 0.33 & 0.45 & 0.15 & 0.35 & 0.54 & 0.64 \\
    & Office & 0.46 & 0.39 & 0.28 & 0.64 & 0.40 & 0.37 & 0.31 & 0.69 & 0.14 & 0.37 & 0.38 & 0.69 & 0.17 & 0.37 & 0.23 & 0.51 & 0.23 & 0.22 & 0.42 & 0.85 \\ \hline
    \rowstyle{\bfseries}& All & 0.43 & 0.26 & 0.33 & 0.74 & 0.34 & 0.26 & 0.36 & 0.77 & 0.19 & 0.22 & 0.31 & 0.77 & 0.22 & 0.30 & 0.27 & 0.60 & 0.19 & 0.15 & 0.23 & 0.79 \\ \midrule
   
   
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}} 
    & Bed & 0.55 & 0.41 & 0.51 & 0.70 & 0.49 & 0.41 & 0.55 & 0.70 & 0.20 & 0.42 & 0.62 & 0.53 & 0.37 & 0.31 & 0.43 & 0.63 & 0.26 & 0.40 & 0.54 & 0.65 \\
    
    & Dishwasher & 0.22 & 0.16 & 0.22 & 0.37 & 0.30 & 0.18 & 0.31 & 0.26 & 0.16 & 0.19 & 0.19 & 0.23 & 0.26 & 0.19 & 0.21 & 0.36 & 0.17 & 0.18 & 0.25 & 0.26 \\
    
    & Door & 0.19 & 0.32 & 0.20 & 0.68 & 0.13 & 0.28 & 0.39 & 0.64 & 0.15 & 0.33 & 0.27 & 0.53 & 0.14 & 0.20 & 0.17 & 0.63 & 0.13 & 0.29 & 0.21 & 0.57 \\
    
    & Mortise lock & 0.12 & 0.14 & 0.09 & 0.35 & 0.14 & 0.23 & 0.11 & 0.46 & 0.07 & 0.29 & 0.12 & 0.35 & 0.16 & 0.18 & 0.15 & 0.47 & 0.09 & 0.27 & 0.22 & 0.53 \\
    
    & Refrigerator & 0.44 & 0.21 & 0.40 & 0.66 & 0.38 & 0.21 & 0.54 & 0.58 & 0.18 & 0.38 & 0.45 & 0.62 & 0.37 & 0.33 & 0.43 & 0.53 & 0.44 & 0.27 & 0.51 & 0.70 \\
    
    & Toilet & 0.18 & 0.16 & 0.29 & 0.37 & 0.25 & 0.16 & 0.26 & 0.49 & 0.22 & 0.34 & 0.41 & 0.47 & 0.34 & 0.26 & 0.42 & 0.56 & 0.24 & 0.23 & 0.25 & 0.51 \\ \hline
    
    \rowstyle{\bfseries} & All & 0.20 & 0.20 & 0.24 & 0.52 & 0.22 & 0.21 & 0.28 & 0.51 & 0.07 & 0.29 & 0.29 & 0.46 & 0.21 & 0.19 & 0.23 & 0.53 & 0.08 & 0.23 & 0.27 & 0.53 \\ \midrule


    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}} 
    & eat & 0.78 & 0.65 & 0.67 & 0.87 & 0.65 & 0.58 & 0.72 & 0.84 & 0.26 & 0.66 & 0.81 & 0.80 & 0.62 & 0.64 & 0.76 & 0.79 & 0.53 & 0.61 & 0.74 & 0.85 \\
    
    & listen to & 0.46 & 0.53 & 0.51 & 0.62 & 0.50 & 0.52 & 0.50 & 0.60 & 0.30 & 0.53 & 0.55 & 0.51 & 0.57 & 0.47 & 0.59 & 0.46 & 0.23 & 0.47 & 0.51 & 0.63 \\
    
    & play & 0.63 & 0.58 & 0.69 & 0.70 & 0.55 & 0.60 & 0.73 & 0.66 & 0.37 & 0.64 & 0.65 & 0.55 & 0.64 & 0.53 & 0.69 & 0.68 & 0.37 & 0.42 & 0.52 & 0.63 \\
    
    & read & 0.42 & 0.46 & 0.65 & 0.73 & 0.30 & 0.42 & 0.66 & 0.78 & 0.26 & 0.29 & 0.59 & 0.57 & 0.41 & 0.43 & 0.63 & 0.68 & 0.31 & 0.19 & 0.57 & 0.64 \\
    
    & wash with & 0.49 & 0.46 & 0.33 & 0.65 & 0.42 & 0.53 & 0.45 & 0.63 & 0.30 & 0.56 & 0.30 & 0.64 & 0.42 & 0.50 & 0.35 & 0.57 & 0.33 & 0.42 & 0.32 & 0.62 \\
    
    & wear & 0.66 & 0.64 & 0.76 & 0.92 & 0.62 & 0.57 & 0.74 & 0.93 & 0.24 & 0.64 & 0.77 & 0.70 & 0.53 & 0.62 & 0.74 & 0.87 & 0.30 & 0.61 & 0.77 & 0.85 \\ \hline

    \rowstyle{\bfseries} & All & 0.53 & 0.53 & 0.38 & 0.74 & 0.37 & 0.50 & 0.44 & 0.74 & 0.20 & 0.55 & 0.37 & 0.62 & 0.49 & 0.51 & 0.37 & 0.67 & 0.15 & 0.40 & 0.26 & 0.70 \\

    \bottomrule
    \end{tabularx}
    \caption{All results of the contextual masked-language models.}
    \label{tab:masked-score-summary}
\end{table*}


\begin{table*}
    \centering
    \setlength{\tabcolsep}{2pt}
    \scriptsize
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X }
    \toprule
    &  & \multicolumn{6}{c}{\textbf{GPT2}} & \multicolumn{6}{c}{\textbf{GPT-Neo}} & \multicolumn{6}{c}{\textbf{GPT-J}} \\ 
    &  & Cos & P-I & P-I-L & P-C & P-C-L & Clas & Cos & P-I & P-I-L & P-C & P-C-L & Clas & Cos & P-I & P-I-L & P-C & P-C-L & Clas  \\ \midrule
    
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}}
    & Bathroom & 0.52 & 0.30 & 0.58 & 0.50 & 0.37 & 0.96 & 0.30 & 0.54 & 0.69 & 0.36 & 0.25 & 0.98 & 0.50 & 0.68 & 0.74 & 0.66 & 0.48 & 0.93 \\
    & Bedroom & 0.26 & 0.26 & 0.27 & 0.47 & 0.38 & 0.57 & 0.19 & 0.53 & 0.44 & 0.53 & 0.48 & 0.72 & 0.24 & 0.49 & 0.34 & 0.62 & 0.48 & 0.71 \\
    & Kitchen & 0.34 & 0.28 & 0.60 & 0.69 & 0.60 & 0.84 & 0.31 & 0.46 & 0.81 & 0.70 & 0.57 & 0.88 & 0.33 & 0.27 & 0.71 & 0.83 & 0.70 & 0.81 \\
    & Living room & 0.21 & 0.40 & 0.45 & 0.41 & 0.33 & 0.43 & 0.26 & 0.62 & 0.67 & 0.60 & 0.44 & 0.63 & 0.21 & 0.60 & 0.70 & 0.67 & 0.45 & 0.65 \\
    & Office & 0.13 & 0.47 & 0.43 & 0.37 & 0.23 & 0.85 & 0.33 & 0.52 & 0.46 & 0.46 & 0.34 & 0.90 & 0.23 & 0.54 & 0.58 & 0.49 & 0.39 & 0.81 \\ \hline
    \rowstyle{\bfseries}& All & 0.26 & 0.27 & 0.46 & 0.46 & 0.35 & 0.74 & 0.15 & 0.48 & 0.62 & 0.44 & 0.35 & 0.83 & 0.23 & 0.48 & 0.61 & 0.56 & 0.41 & 0.78 \\ \midrule
   
   
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}}
    & Bed & 0.36 & 0.52 & 0.68 & 0.67 & 0.45 & 0.63 & 0.32 & 0.61 & 0.65 & 0.77 & 0.70 & 0.80 & 0.46 & 0.63 & 0.68 & 0.81 & 0.68 & 0.73 \\
    
    & Dishwasher & 0.11 & 0.34 & 0.43 & 0.25 & 0.23 & 0.33 & 0.06 & 0.45 & 0.50 & 0.30 & 0.29 & 0.25 & 0.09 & 0.49 & 0.51 & 0.44 & 0.38 & 0.35 \\
    
    & Door & 0.23 & 0.12 & 0.24 & 0.20 & 0.28 & 0.58 & 0.27 & 0.23 & 0.27 & 0.35 & 0.42 & 0.66 & 0.15 & 0.34 & 0.37 & 0.37 & 0.41 & 0.72 \\
    
    & Mortise lock & 0.07 & 0.39 & 0.44 & 0.17 & 0.18 & 0.54 & 0.11 & 0.46 & 0.52 & 0.30 & 0.22 & 0.60 & 0.15 & 0.52 & 0.51 & 0.47 & 0.31 & 0.57 \\
    
    & Refrigerator & 0.42 & 0.57 & 0.30 & 0.53 & 0.52 & 0.64 & 0.29 & 0.44 & 0.40 & 0.47 & 0.55 & 0.64 & 0.46 & 0.45 & 0.42 & 0.57 & 0.63 & 0.62 \\
    
    & Toilet & 0.29 & 0.31 & 0.42 & 0.20 & 0.17 & 0.57 & 0.27 & 0.50 & 0.57 & 0.25 & 0.26 & 0.52 & 0.32 & 0.45 & 0.55 & 0.32 & 0.37 & 0.59 \\\hline
    
    \rowstyle{\bfseries}& All & 0.14 & 0.34 & 0.39 & 0.28 & 0.25 & 0.55 & 0.12 & 0.44 & 0.47 & 0.37 & 0.36 & 0.57 & 0.16 & 0.47 & 0.49 & 0.42 & 0.43 & 0.59 \\ \midrule
    
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}} 
    & eat & 0.49 & 0.82 & 0.65 & - & - & 0.84 & 0.45 & 0.86 & 0.66 & - & - & 0.86 & 0.48 & 0.68 & 0.74 & - & - & 0.90 \\
    
    & listen to & 0.22 & 0.57 & 0.51 & - & - & 0.57 & 0.22 & 0.47 & 0.47 & - & - & 0.49 & 0.21 & 0.60 & 0.56 & - & - & 0.57 \\
    
    & play & 0.40 & 0.64 & 0.62 & - & - & 0.61 & 0.32 & 0.66 & 0.61 & - & - & 0.59 & 0.34 & 0.66 & 0.70 & - & - & 0.68 \\
    
    & read & 0.32 & 0.63 & 0.30 & - & - & 0.51 & 0.32 & 0.61 & 0.34 & - & - & 0.46 & 0.40 & 0.63 & 0.41 & - & - & 0.60 \\
    
    & wash with & 0.39 & 0.77 & 0.51 & - & - & 0.57 & 0.28 & 0.66 & 0.52 & - & - & 0.57 & 0.23 & 0.69 & 0.52 & - & - & 0.65 \\
    
    & wear & 0.44 & 0.38 & 0.72 & - & - & 0.85 & 0.16 & 0.39 & 0.66 & - & - & 0.83 & 0.21 & 0.38 & 0.62 & - & - & 0.87 \\ \midrule
    
    \rowstyle{\bfseries}& All & 0.31 & 0.52 & 0.53 & - & - & 0.66 & 0.19 & 0.49 & 0.52 & - & - & 0.63 & 0.23 & 0.50 & 0.56 & - & - & 0.71 \\ \bottomrule

    \end{tabularx}
    \caption{All results of the contextual causal-language models.}
    \label{tab:gpt-score-summary}
\end{table*}

==> tabellen/tab_score_summary_v3.tex <==
\begin{table*}
    \setlength{\tabcolsep}{2pt}
    \centering
    \tiny
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X }
    \toprule
    &  & \multicolumn{6}{c}{\textbf{Word2Vec}} & \multicolumn{6}{c}{\textbf{GloVe}} & \multicolumn{6}{c}{\textbf{Levy}} & \multicolumn{6}{c}{\textbf{fastText}}\\ 
    &  & cos & dist & kend & knn & svm & ffn & cos & dist & kend & knn & svm & ffn & cos & dist & kend & knn & svm & ffn & cos & dist & kend & knn & svm & ffn \\ \midrule
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}} 
    & bathroom & 0.34 & 0.37 & 0.37 & 0.66 & 0.62 & 0.81 & 0.35 & 0.38 & 0.37 & 0.74 & 0.95 & 0.97 & 0.33 & 0.38 & 0.37 & 0.12 & 0.35 & 0.35 & 0.45 & 0.51 & 0.50 & 0.71 & 0.74 & 0.99 \\
    
    & bedroom & 0.21 & 0.21 & 0.21 & 0.36 & 0.53 & 0.68 & 0.31 & 0.29 & 0.31 & 0.38 & 0.48 & 0.56 & 0.18 & 0.20 & 0.20 & 0.07 & 0.25 & 0.13 & 0.29 & 0.31 & 0.31 & 0.20 & 0.39 & 0.53 \\
    
    & kitchen & 0.37 & 0.36 & 0.36 & 0.45 & 0.54 & 0.61 & 0.40 & 0.42 & 0.43 & 0.48 & 0.76 & 0.73 & 0.15 & 0.17 & 0.17 & 0.05 & 0.27 & 0.30 & 0.33 & 0.35 & 0.34 & 0.42 & 0.73 & 0.84 \\
    
    & living room & 0.36 & 0.22 & 0.21 & 0.22 & 0.45 & 0.47 & 0.27 & 0.27 & 0.26 & 0.09 & 0.46 & 0.52 & 0.16 & 0.23 & 0.23 & 0.08 & 0.10 & 0.17 & 0.18 & 0.26 & 0.27 & 0.28 & 0.21 & 0.69 \\
    
    & office & 0.24 & 0.22 & 0.21 & 0.66 & 0.59 & 0.63 & 0.17 & 0.35 & 0.37 & 0.73 & 0.73 & 0.69 & 0.26 & 0.27 & 0.28 & 0.35 & 0.42 & 0.43 & 0.34 & 0.34 & 0.36 & 0.68 & 0.41 & 0.62 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.24 & 0.23 & 0.23 & 0.47 & 0.55 & 0.63 & 0.26 & 0.32 & 0.33 & 0.49 & 0.67 & 0.70 & 0.14 & 0.15 & 0.15 & 0.11 & 0.13 & 0.25 & 0.26 & 0.31 & 0.31 & 0.45 & 0.48 & 0.74 \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}} 
    & bed & 0.42 & 0.43 & 0.41 & 0.47 & 0.43 & 0.53 & 0.41 & 0.50 & 0.48 & 0.59 & 0.73 & 0.86 & - & - & - & - & - & - & 0.52 & 0.53 & 0.53 & 0.44 & 0.53 & 0.78 \\
    
    & dishwasher & 0.20 & 0.24 & 0.24 & 0.23 & 0.34 & 0.28 & 0.32 & 0.31 & 0.30 & 0.15 & 0.17 & 0.24 & - & - & - & - & - & - & 0.36 & 0.31 & 0.31 & 0.11 & 0.12 & 0.30 \\
    
    & door & 0.12 & 0.11 & 0.12 & 0.38 & 0.70 & 0.74 & 0.17 & 0.21 & 0.22 & 0.44 & 0.85 & 0.80 & - & - & - & - & - & - & 0.21 & 0.25 & 0.23 & 0.54 & 0.57 & 0.75 \\
    
    & mortise lock & 0.13 & 0.18 & 0.20 & 0.40 & 0.36 & 0.41 & 0.11 & 0.28 & 0.29 & 0.23 & 0.65 & 0.52 & - & - & - & - & - & - & 0.12 & 0.17 & 0.19 & 0.33 & 0.39 & 0.63 \\

    & refrigerator & 0.36 & 0.42 & 0.41 & 0.40 & 0.45 & 0.48 & 0.52 & 0.56 & 0.55 & 0.58 & 0.62 & 0.71 & - & - & - & - & - & - & 0.51 & 0.58 & 0.58 & 0.26 & 0.41 & 0.50 \\
    
    & toilet & 0.22 & 0.26 & 0.26 & 0.24 & 0.55 & 0.50 & 0.26 & 0.32 & 0.30 & 0.35 & 0.51 & 0.53 & - & - & - & - & - & - & 0.32 & 0.35 & 0.34 & 0.50 & 0.65 & 0.78 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.16 & 0.27 & 0.26 & 0.34 & 0.48 & 0.50 & 0.23 & 0.34 & 0.34 & 0.39 & 0.59 & 0.61 & - & - & - & - & - & - & 0.24 & 0.34 & 0.34 & 0.33 & 0.45 & 0.61 \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}} 
    & eat & 0.79 & 0.79 & 0.77 & 0.89 & 0.89 & 0.89 & 0.77 & 0.86 & 0.80 & 0.85 & 0.89 & 0.92 & 0.45 & 0.44 & 0.45 & 0.83 & 0.87 & 0.87 & 0.75 & 0.80 & 0.79 & 0.66 & 0.89 & 0.89 \\
    
    & listen to & 0.56 & 0.66 & 0.58 & 0.37 & 0.38 & 0.42 & 0.49 & 0.71 & 0.66 & 0.30 & 0.53 & 0.49 & 0.31 & 0.30 & 0.30 & 0.11 & 0.41 & 0.51 & 0.34 & 0.47 & 0.54 & 0.54 & 0.42 & 0.38 \\
    
    & play & 0.65 & 0.70 & 0.64 & 0.50 & 0.66 & 0.59 & 0.65 & 0.80 & 0.72 & 0.35 & 0.42 & 0.43 & 0.45 & 0.45 & 0.44 & 0.64 & 0.50 & 0.56 & 0.64 & 0.70 & 0.69 & 0.60 & 0.66 & 0.65 \\
    
    & read & 0.42 & 0.52 & 0.48 & 0.46 & 0.55 & 0.61 & 0.50 & 0.60 & 0.58 & 0.44 & 0.41 & 0.48 & 0.34 & 0.32 & 0.32 & 0.47 & 0.39 & 0.53 & 0.53 & 0.56 & 0.59 & 0.47 & 0.50 & 0.56 \\
    
    & wash with & 0.42 & 0.52 & 0.51 & 0.48 & 0.66 & 0.63 & 0.45 & 0.57 & 0.52 & 0.61 & 0.66 & 0.62 & 0.35 & 0.32 & 0.33 & 0.47 & 0.66 & 0.60 & 0.33 & 0.52 & 0.51 & 0.62 & 0.66 & 0.66 \\
    
    & wear & 0.76 & 0.78 & 0.76 & 0.88 & 0.84 & 0.87 & 0.81 & 0.87 & 0.84 & 0.88 & 0.88 & 0.85 & 0.59 & 0.55 & 0.52 & 0.79 & 0.85 & 0.85 & 0.79 & 0.81 & 0.79 & 0.69 & 0.93 & 0.93 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.55 & 0.60 & 0.57 & 0.58 & 0.64 & 0.66 & 0.58 & 0.68 & 0.64 & 0.55 & 0.63 & 0.64 & 0.35 & 0.33 & 0.33 & 0.56 & 0.61 & 0.65 & 0.48 & 0.58 & 0.57 & 0.51 & 0.66 & 0.67 \\
    \bottomrule
    \end{tabularx}
    \caption{All results of the static models. cos: Cosine Measure, dist: Distance Correlation, kend: Kendall's Tau, knn: K-Nearest Neighbors, svm: Support Vector Machine, fnn: Feed-Forward Network. The gap in Levy is due to its small training set, because of which it did not know many of the words in our study.}
    \label{tab:static-score-summary}
\end{table*}



\begin{table*}
    \centering
    \setlength{\tabcolsep}{2pt}
    \tiny
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X}
    \toprule
    &  & \multicolumn{6}{c}{\textbf{BERT-Base}} & \multicolumn{6}{c}{\textbf{BERT-Large}} & \multicolumn{6}{c}{\textbf{RoBERTa}} & \multicolumn{6}{c}{\textbf{ElectraGen}} & \multicolumn{6}{c}{\textbf{Albert}} \\ 
    &  & cos & m-s & m-t & knn & svm & ffn & cos & m-s & m-t & knn & svm & ffn & cos & m-s & m-t & knn & svm & ffn & cos & m-s & m-t & knn & svm & ffn & cos & m-s & m-t & knn & svm & ffn \\ \midrule
    
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}} 
    & bathroom & 0.57 & 0.13 & 0.52 & 0.72 & 0.87 & 0.93 & 0.65 & 0.30 & 0.59 & 0.78 & 0.93 & 0.93 & 0.21 & 0.24 & 0.52 & 0.55 & 0.83 & 0.88 & 0.58 & 0.32 & 0.34 & 0.49 & 0.72 & 0.73 & 0.24 & 0.18 & 0.39 & 0.52 & 0.75 & 0.90 \\
    
    & bedroom & 0.48 & 0.33 & 0.43 & 0.53 & 0.66 & 0.77 & 0.44 & 0.41 & 0.44 & 0.44 & 0.87 & 0.78 & 0.23 & 0.18 & 0.36 & 0.17 & 0.53 & 0.60 & 0.32 & 0.31 & 0.37 & 0.37 & 0.37 & 0.39 & 0.23 & 0.22 & 0.47 & 0.31 & 0.44 & 0.68 \\
    
    & kitchen & 0.56 & 0.25 & 0.58 & 0.62 & 0.81 & 0.83 & 0.43 & 0.24 & 0.54 & 0.72 & 0.77 & 0.79 & 0.39 & 0.27 & 0.59 & 0.16 & 0.62 & 0.73 & 0.34 & 0.24 & 0.36 & 0.48 & 0.34 & 0.39 & 0.25 & 0.17 & 0.30 & 0.05 & 0.56 & 0.69 \\
    
    & living room & 0.30 & 0.37 & 0.26 & 0.51 & 0.78 & 0.79 & 0.23 & 0.38 & 0.24 & 0.57 & 0.49 & 0.66 & 0.13 & 0.38 & 0.28 & 0.49 & 0.74 & 0.65 & 0.26 & 0.48 & 0.33 & 0.15 & 0.27 & 0.26 & 0.15 & 0.35 & 0.54 & 0.20 & 0.29 & 0.40 \\
    
    & office & 0.46 & 0.39 & 0.28 & 0.40 & 0.59 & 0.61 & 0.40 & 0.37 & 0.31 & 0.25 & 0.52 & 0.71 & 0.14 & 0.37 & 0.38 & 0.18 & 0.74 & 0.63 & 0.17 & 0.37 & 0.23 & 0.42 & 0.27 & 0.36 & 0.23 & 0.22 & 0.42 & 0.45 & 0.66 & 0.81 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.43 & 0.26 & 0.33 & 0.54 & 0.73 & 0.78 & 0.34 & 0.26 & 0.36 & 0.55 & 0.72 & 0.78 & 0.19 & 0.22 & 0.31 & 0.28 & 0.69 & 0.71 & 0.22 & 0.30 & 0.27 & 0.38 & 0.40 & 0.43 & 0.19 & 0.15 & 0.23 & 0.25 & 0.53 & 0.69 \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}} 
    & bed & 0.55 & 0.41 & 0.51 & 0.51 & 0.69 & 0.79 & 0.49 & 0.41 & 0.55 & 0.56 & 0.69 & 0.69 & 0.20 & 0.42 & 0.62 & 0.49 & 0.52 & 0.60 & 0.37 & 0.31 & 0.43 & 0.44 & 0.44 & 0.43 & 0.26 & 0.40 & 0.54 & 0.36 & 0.66 & 0.71 \\
    
    & dishwasher & 0.22 & 0.16 & 0.22 & 0.27 & 0.31 & 0.28 & 0.30 & 0.18 & 0.31 & 0.29 & 0.17 & 0.18 & 0.16 & 0.19 & 0.19 & 0.13 & 0.24 & 0.17 & 0.26 & 0.19 & 0.21 & 0.01 & 0.23 & 0.36 & 0.17 & 0.18 & 0.25 & 0.26 & 0.25 & 0.23 \\
    
    & door & 0.19 & 0.32 & 0.20 & 0.34 & 0.65 & 0.63 & 0.13 & 0.28 & 0.39 & 0.47 & 0.60 & 0.62 & 0.15 & 0.33 & 0.27 & 0.52 & 0.42 & 0.51 & 0.14 & 0.20 & 0.17 & 0.41 & 0.57 & 0.60 & 0.13 & 0.29 & 0.21 & 0.36 & 0.50 & 0.54 \\
    
    & mortise lock & 0.12 & 0.14 & 0.09 & 0.16 & 0.26 & 0.28 & 0.14 & 0.23 & 0.11 & 0.19 & 0.26 & 0.35 & 0.07 & 0.29 & 0.12 & 0.08 & 0.18 & 0.28 & 0.16 & 0.18 & 0.15 & 0.39 & 0.59 & 0.39 & 0.09 & 0.27 & 0.22 & 0.16 & 0.31 & 0.39 \\
    
    & refrigerator & 0.44 & 0.21 & 0.40 & 0.48 & 0.47 & 0.54 & 0.38 & 0.21 & 0.54 & 0.42 & 0.51 & 0.50 & 0.18 & 0.38 & 0.45 & 0.49 & 0.43 & 0.49 & 0.37 & 0.33 & 0.43 & 0.46 & 0.45 & 0.53 & 0.44 & 0.27 & 0.51 & 0.66 & 0.51 & 0.61 \\
    
    & toilet & 0.18 & 0.16 & 0.29 & 0.16 & 0.34 & 0.45 & 0.25 & 0.16 & 0.26 & 0.36 & 0.55 & 0.50 & 0.22 & 0.34 & 0.41 & 0.45 & 0.51 & 0.51 & 0.34 & 0.26 & 0.42 & 0.26 & 0.41 & 0.46 & 0.24 & 0.23 & 0.25 & 0.22 & 0.31 & 0.46 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.20 & 0.20 & 0.24 & 0.33 & 0.45 & 0.49 & 0.22 & 0.21 & 0.28 & 0.39 & 0.46 & 0.46 & 0.07 & 0.29 & 0.29 & 0.39 & 0.39 & 0.43 & 0.21 & 0.19 & 0.23 & 0.32 & 0.45 & 0.47 & 0.08 & 0.23 & 0.27 & 0.35 & 0.42 & 0.49 \\ \midrule
    
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}} 
    & eat & 0.78 & 0.65 & 0.67 & 0.89 & 0.84 & 0.90 & 0.65 & 0.58 & 0.72 & 0.80 & 0.89 & 0.90 & 0.26 & 0.66 & 0.81 & 0.65 & 0.87 & 0.86 & 0.62 & 0.64 & 0.76 & 0.74 & 0.79 & 0.79 & 0.53 & 0.61 & 0.74 & 0.57 & 0.84 & 0.85 \\
    
    & listen to & 0.46 & 0.53 & 0.51 & 0.42 & 0.52 & 0.57 & 0.50 & 0.52 & 0.50 & 0.43 & 0.55 & 0.52 & 0.30 & 0.53 & 0.55 & 0.23 & 0.49 & 0.54 & 0.57 & 0.47 & 0.59 & 0.00 & 0.36 & 0.39 & 0.23 & 0.47 & 0.51 & 0.07 & 0.44 & 0.57 \\
    
    & play & 0.63 & 0.58 & 0.69 & 0.54 & 0.58 & 0.61 & 0.55 & 0.60 & 0.73 & 0.54 & 0.64 & 0.66 & 0.37 & 0.64 & 0.65 & 0.38 & 0.53 & 0.59 & 0.64 & 0.53 & 0.69 & 0.64 & 0.64 & 0.65 & 0.37 & 0.42 & 0.52 & 0.45 & 0.60 & 0.62 \\
    
    & read & 0.42 & 0.46 & 0.65 & 0.34 & 0.73 & 0.65 & 0.30 & 0.42 & 0.66 & 0.42 & 0.77 & 0.59 & 0.26 & 0.29 & 0.59 & 0.21 & 0.44 & 0.44 & 0.41 & 0.43 & 0.63 & 0.51 & 0.68 & 0.69 & 0.31 & 0.19 & 0.57 & 0.35 & 0.63 & 0.60 \\
    
    & wash with & 0.49 & 0.46 & 0.33 & 0.49 & 0.66 & 0.63 & 0.42 & 0.53 & 0.45 & 0.61 & 0.62 & 0.60 & 0.30 & 0.56 & 0.30 & 0.23 & 0.60 & 0.59 & 0.42 & 0.50 & 0.35 & 0.52 & 0.40 & 0.41 & 0.33 & 0.42 & 0.32 & 0.18 & 0.46 & 0.51 \\

    & wear & 0.66 & 0.64 & 0.76 & 0.88 & 0.90 & 0.92 & 0.62 & 0.57 & 0.74 & 0.79 & 0.90 & 0.85 & 0.24 & 0.64 & 0.77 & 0.36 & 0.72 & 0.79 & 0.53 & 0.62 & 0.74 & 0.90 & 0.84 & 0.83 & 0.30 & 0.61 & 0.77 & 0.61 & 0.77 & 0.86 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.53 & 0.53 & 0.38 & 0.59 & 0.69 & 0.71 & 0.37 & 0.50 & 0.44 & 0.60 & 0.73 & 0.68 & 0.20 & 0.55 & 0.37 & 0.28 & 0.59 & 0.64 & 0.49 & 0.51 & 0.37 & 0.60 & 0.61 & 0.62 & 0.15 & 0.40 & 0.26 & 0.29 & 0.62 & 0.67 \\
    
    \bottomrule
    \end{tabularx}
    \caption{All results of the contextual masked-language models. cos: Cosine Measure, m-s: Masked-Source Log Score, m-t: Masked-Target Log Score, knn: K-Nearest Neighbors, svm: Support Vector Machine, fnn: Feed-Forward Network.}
    \label{tab:masked-score-summary}
\end{table*}


\begin{table*}
    \centering
    \setlength{\tabcolsep}{2pt}
    \tiny
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X ^X ^X }
    \toprule
    &  & \multicolumn{8}{c}{\textbf{GPT2}} & \multicolumn{8}{c}{\textbf{GPT-Neo}} & \multicolumn{8}{c}{\textbf{GPT-J}} \\ 
    &  & cos & p-s & p-s-l & p-t & p-t-l & knn & svm & ffn & cos & p-s & p-s-l & p-t & p-t-l & knn & svm & ffn & cos & p-s & p-s-l & p-t & p-t-l & knn & svm & ffn  \\ \midrule
    
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}}
    & bathroom & 0.52 & 0.20 & 0.38 & 0.50 & 0.37 & 0.31 & 0.95 & 0.95 & 0.30 & 0.22 & 0.51 & 0.36 & 0.25 & 0.53 & 0.89 & 0.91 & 0.50 & 0.26 & 0.60 & 0.66 & 0.48 & 0.35 & 0.89 & 0.92 \\
    
    & bedroom & 0.26 & 0.31 & 0.23 & 0.47 & 0.38 & 0.26 & 0.61 & 0.54 & 0.19 & 0.33 & 0.21 & 0.53 & 0.48 & 0.55 & 0.49 & 0.57 & 0.24 & 0.32 & 0.23 & 0.62 & 0.48 & 0.33 & 0.70 & 0.64 \\
    
    & kitchen & 0.34 & 0.41 & 0.45 & 0.69 & 0.60 & 0.53 & 0.82 & 0.83 & 0.31 & 0.49 & 0.67 & 0.70 & 0.57 & 0.38 & 0.51 & 0.81 & 0.33 & 0.36 & 0.52 & 0.83 & 0.70 & 0.70 & 0.82 & 0.83 \\
    
    & living room & 0.21 & 0.43 & 0.26 & 0.41 & 0.33 & 0.16 & 0.27 & 0.46 & 0.26 & 0.57 & 0.39 & 0.60 & 0.44 & 0.28 & 0.13 & 0.48 & 0.21 & 0.50 & 0.47 & 0.67 & 0.45 & 0.46 & 0.40 & 0.63 \\
    
    & office & 0.13 & 0.21 & 0.43 & 0.37 & 0.23 & 0.31 & 0.44 & 0.73 & 0.33 & 0.30 & 0.43 & 0.46 & 0.34 & 0.24 & 0.53 & 0.72 & 0.23 & 0.36 & 0.53 & 0.49 & 0.39 & 0.37 & 0.52 & 0.69 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.26 & 0.23 & 0.30 & 0.46 & 0.35 & 0.30 & 0.61 & 0.72 & 0.15 & 0.34 & 0.44 & 0.44 & 0.35 & 0.40 & 0.52 & 0.71 & 0.23 & 0.32 & 0.42 & 0.56 & 0.41 & 0.42 & 0.66 & 0.74 \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}}
    & bed & 0.36 & 0.30 & 0.51 & 0.67 & 0.45 & 0.55 & 0.59 & 0.70 & 0.32 & 0.38 & 0.46 & 0.77 & 0.70 & 0.66 & 0.78 & 0.88 & 0.46 & 0.38 & 0.36 & 0.81 & 0.68 & 0.71 & 0.83 & 0.84 \\
    
    & dishwasher & 0.11 & 0.34 & 0.22 & 0.25 & 0.23 & 0.18 & 0.21 & 0.28 & 0.06 & 0.23 & 0.30 & 0.30 & 0.29 & 0.15 & 0.15 & 0.24 & 0.09 & 0.26 & 0.30 & 0.44 & 0.38 & 0.12 & 0.15 & 0.32 \\
    
    & door & 0.23 & 0.07 & 0.14 & 0.20 & 0.28 & 0.20 & 0.65 & 0.66 & 0.27 & 0.10 & 0.17 & 0.35 & 0.42 & 0.20 & 0.44 & 0.66 & 0.15 & 0.13 & 0.12 & 0.37 & 0.41 & 0.25 & 0.67 & 0.77 \\
    
    & mortise lock & 0.07 & 0.34 & 0.43 & 0.17 & 0.18 & 0.27 & 0.63 & 0.65 & 0.11 & 0.49 & 0.42 & 0.30 & 0.22 & 0.27 & 0.49 & 0.61 & 0.15 & 0.43 & 0.43 & 0.47 & 0.31 & 0.04 & 0.63 & 0.66 \\
    
    & refrigerator & 0.42 & 0.41 & 0.24 & 0.53 & 0.52 & 0.47 & 0.39 & 0.51 & 0.29 & 0.33 & 0.33 & 0.47 & 0.55 & 0.44 & 0.47 & 0.57 & 0.46 & 0.51 & 0.41 & 0.57 & 0.63 & 0.55 & 0.53 & 0.63 \\
    
    & toilet & 0.29 & 0.36 & 0.44 & 0.20 & 0.17 & 0.16 & 0.49 & 0.54 & 0.27 & 0.42 & 0.50 & 0.25 & 0.26 & 0.23 & 0.50 & 0.58 & 0.32 & 0.45 & 0.48 & 0.32 & 0.37 & 0.26 & 0.53 & 0.62 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.14 & 0.24 & 0.28 & 0.28 & 0.25 & 0.29 & 0.47 & 0.54 & 0.12 & 0.30 & 0.34 & 0.37 & 0.36 & 0.32 & 0.46 & 0.57 & 0.16 & 0.34 & 0.32 & 0.42 & 0.43 & 0.33 & 0.54 & 0.62 \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}}
    & eat & 0.49 & 0.82 & 0.65 & - & - & 0.82 & 0.87 & 0.87 & 0.45 & 0.86 & 0.66 & - & - & 0.76 & 0.87 & 0.88 & 0.48 & 0.68 & 0.74 & - & - & 0.63 & 0.89 & 0.89 \\
    
    & listen to & 0.22 & 0.57 & 0.51 & - & - & 0.29 & 0.50 & 0.58 & 0.22 & 0.47 & 0.47 & - & - & 0.20 & 0.42 & 0.55 & 0.21 & 0.60 & 0.56 & - & - & 0.29 & 0.52 & 0.60 \\
    
    & play & 0.40 & 0.64 & 0.62 & - & - & 0.62 & 0.61 & 0.59 & 0.32 & 0.66 & 0.61 & - & - & 0.20 & 0.55 & 0.62 & 0.34 & 0.66 & 0.70 & - & - & 0.37 & 0.67 & 0.67 \\
    
    & read & 0.32 & 0.63 & 0.30 & - & - & 0.32 & 0.45 & 0.45 & 0.32 & 0.61 & 0.34 & - & - & 0.29 & 0.52 & 0.49 & 0.40 & 0.63 & 0.41 & - & - & 0.20 & 0.59 & 0.49 \\
    
    & Wash with & 0.39 & 0.77 & 0.51 & - & - & 0.57 & 0.61 & 0.63 & 0.28 & 0.66 & 0.52 & - & - & 0.39 & 0.41 & 0.60 & 0.23 & 0.69 & 0.52 & - & - & 0.66 & 0.61 & 0.64 \\
    
    & wear & 0.44 & 0.38 & 0.72 & - & - & 0.76 & 0.84 & 0.87 & 0.16 & 0.39 & 0.66 & - & - & 0.68 & 0.79 & 0.85 & 0.21 & 0.38 & 0.62 & - & - & 0.87 & 0.84 & 0.87 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.31 & 0.52 & 0.53 & - & - & 0.51 & 0.64 & 0.66 & 0.19 & 0.49 & 0.52 & - & - & 0.40 & 0.59 & 0.66 & 0.23 & 0.50 & 0.56 & - & - & 0.48 & 0.68 & 0.69 \\

    \bottomrule
    \end{tabularx}
    \caption{All results of the contextual causal-language models. p-s: Predict Source Score, p-s-l: : Predict Source Log Score, p-t: Predict Target Score, p-t-l: Predict Target Log Score. The gap for the verb p-t score is due to the lack of an easily applicable sentence templates in this direction.}
    \label{tab:gpt-score-summary}
\end{table*}

==> tabellen/tab_score_summary_v4_old.tex <==
\begin{table*}
    \setlength{\tabcolsep}{2pt}
    \centering
    \tiny
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X }
    \toprule
    &  & \multicolumn{6}{c}{\textbf{Word2Vec}} & \multicolumn{6}{c}{\textbf{GloVe}} & \multicolumn{6}{c}{\textbf{Levy}} & \multicolumn{6}{c}{\textbf{fastText}}\\ 
    &  & cos & dist & kend & knn & svm & ffn & cos & dist & kend & knn & svm & ffn & cos & dist & kend & knn & svm & ffn & cos & dist & kend & knn & svm & ffn \\ \midrule
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}} 
    & bathroom & 0.34 & 0.37 & 0.37 & 0.66* & 0.62* & 0.81* & 0.35 & 0.38 & 0.37 & 0.74* & 0.95* & 0.97* & 0.33 & 0.38 & 0.37 & 0.12 & 0.35* & 0.35 & 0.45* & 0.51* & 0.50* & 0.71* & 0.74* & 0.99* \\
    
    & bedroom & 0.21 & 0.21 & 0.21 & 0.36* & 0.53* & 0.68* & 0.31 & 0.29 & 0.31 & 0.38* & 0.48* & 0.56* & 0.18 & 0.20 & 0.20 & 0.07 & 0.25 & 0.13 & 0.29 & 0.31 & 0.31 & 0.20 & 0.39* & 0.53* \\
    
    & kitchen & 0.37 & 0.36 & 0.36 & 0.45* & 0.54* & 0.61* & 0.40* & 0.42* & 0.43* & 0.48* & 0.76* & 0.73* & 0.15 & 0.17 & 0.17 & 0.05 & 0.27 & 0.30 & 0.33 & 0.35 & 0.34 & 0.42* & 0.73* & 0.84* \\
    
    & living room & 0.36 & 0.22 & 0.21 & 0.22 & 0.45* & 0.47* & 0.27 & 0.27 & 0.26 & 0.09 & 0.46* & 0.52* & 0.16 & 0.23 & 0.23 & 0.08 & 0.10 & 0.17 & 0.18 & 0.26 & 0.27 & 0.28 & 0.21 & 0.69* \\
    
    & office & 0.24 & 0.22 & 0.21 & 0.66* & 0.59* & 0.63* & 0.17 & 0.35 & 0.37 & 0.73* & 0.73* & 0.69* & 0.26 & 0.27 & 0.28 & 0.35 & 0.42 & 0.43* & 0.34 & 0.34 & 0.36 & 0.68* & 0.41* & 0.62*
 \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.24* & 0.23* & 0.23* & 0.47* & 0.55* & 0.63* & 0.26* & 0.32* & 0.33* & 0.49* & 0.67* & 0.70* & 0.14 & 0.15 & 0.15 & 0.11 & 0.13 & 0.25* & 0.26* & 0.31* & 0.31* & 0.45* & 0.48* & 0.74* \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}} 
    & bed & 0.42* & 0.43* & 0.41* & 0.47* & 0.43* & 0.53* & 0.41* & 0.50* & 0.48* & 0.59* & 0.73* & 0.86* & - & - & - & - & - & - & 0.52* & 0.53* & 0.53* & 0.44* & 0.53* & 0.78* \\
    
    & dishwasher & 0.20 & 0.24 & 0.24 & 0.23 & 0.34* & 0.28 & 0.32* & 0.31* & 0.30* & 0.15 & 0.17 & 0.24 & - & - & - & - & - & - & 0.36* & 0.31* & 0.31* & 0.11 & 0.12 & 0.30* \\
    
    & door & 0.12 & 0.11 & 0.12 & 0.38* & 0.70* & 0.74* & 0.17 & 0.21 & 0.22 & 0.44* & 0.85* & 0.80* & - & - & - & - & - & - & 0.21 & 0.25 & 0.23 & 0.54* & 0.57* & 0.75* \\
    
    & mortise lock & 0.13 & 0.18 & 0.20 & 0.40* & 0.36* & 0.41* & 0.11 & 0.28* & 0.29* & 0.23 & 0.65* & 0.52* & - & - & - & - & - & - & 0.12 & 0.17 & 0.19 & 0.33* & 0.39* & 0.63* \\

    & refrigerator & 0.36* & 0.42* & 0.41* & 0.40* & 0.45* & 0.48* & 0.52* & 0.56* & 0.55* & 0.58* & 0.62* & 0.71* & - & - & - & - & - & - & 0.51* & 0.58* & 0.58* & 0.26 & 0.41* & 0.50* \\
    
    & toilet & 0.22 & 0.26 & 0.26 & 0.24 & 0.55* & 0.50* & 0.26 & 0.32* & 0.30* & 0.35* & 0.51* & 0.53* & - & - & - & - & - & - & 0.32* & 0.35* & 0.34* & 0.50* & 0.65* & 0.78* \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.16* & 0.27* & 0.26* & 0.34* & 0.48* & 0.50* & 0.23* & 0.34* & 0.34* & 0.39* & 0.59* & 0.61* & - & - & - & - & - & - & 0.24* & 0.34* & 0.34* & 0.33* & 0.45* & 0.61* \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}} 
    & eat & 0.79* & 0.79* & 0.77* & 0.89* & 0.89* & 0.89* & 0.77* & 0.86* & 0.80* & 0.85* & 0.89* & 0.92* & 0.45* & 0.44* & 0.45* & 0.83* & 0.87* & 0.87* & 0.75* & 0.80* & 0.79* & 0.66* & 0.89* & 0.89* \\
    
    & listen to & 0.56* & 0.66* & 0.58* & 0.37* & 0.38* & 0.42* & 0.49* & 0.71* & 0.66* & 0.30 & 0.53* & 0.49* & 0.31 & 0.30 & 0.30 & 0.11 & 0.41* & 0.51* & 0.34* & 0.47* & 0.54* & 0.54* & 0.42* & 0.38* \\
    
    & play & 0.65* & 0.70* & 0.64* & 0.50* & 0.66* & 0.59* & 0.65* & 0.80* & 0.72* & 0.35 & 0.42* & 0.43* & 0.45* & 0.45* & 0.44* & 0.64* & 0.50* & 0.56* & 0.64* & 0.70* & 0.69* & 0.60 & 0.66* & 0.65* \\
    
    & read & 0.42* & 0.52* & 0.48* & 0.46* & 0.55* & 0.61* & 0.50* & 0.60* & 0.58* & 0.44* & 0.41* & 0.48* & 0.34 & 0.32 & 0.32 & 0.47* & 0.39* & 0.53* & 0.53* & 0.56* & 0.59* & 0.47* & 0.50* & 0.56* \\
    
    & wash with & 0.42* & 0.52* & 0.51* & 0.48* & 0.66* & 0.63* & 0.45* & 0.57* & 0.52* & 0.61* & 0.66* & 0.62* & 0.35 & 0.32 & 0.33 & 0.47* & 0.66* & 0.60* & 0.33 & 0.52* & 0.51* & 0.62* & 0.66* & 0.66* \\
    
    & wear & 0.76* & 0.78* & 0.76* & 0.88* & 0.84* & 0.87* & 0.81* & 0.87* & 0.84* & 0.88* & 0.88* & 0.85* & 0.59* & 0.55* & 0.52* & 0.79* & 0.85* & 0.85* & 0.79* & 0.81* & 0.79* & 0.69* & 0.93* & 0.93* \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.55* & 0.60* & 0.57* & 0.58* & 0.64* & 0.66* & 0.58* & 0.68* & 0.64* & 0.55* & 0.63* & 0.64* & 0.35* & 0.33* & 0.33* & 0.56* & 0.61* & 0.65* & 0.48* & 0.58* & 0.57* & 0.51* & 0.66* & 0.67* \\
    \bottomrule
    \end{tabularx}
    \caption{All results of the static models. cos: Cosine Measure, dist: Distance Correlation, kend: Kendall's Tau, knn: K-Nearest Neighbors, svm: Support Vector Machine, fnn: Feed-Forward Network. The gap in Levy is due to its small training set and the corresponding small vocabulary. \T{(* indicates significant at p < 0.01)}}
    \label{tab:static-score-summary}
\end{table*}



\begin{table*}
    \centering
    \setlength{\tabcolsep}{2pt}
    \tiny
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X}
    \toprule
    &  & \multicolumn{6}{c}{\textbf{BERT-Base}} & \multicolumn{6}{c}{\textbf{BERT-Large}} & \multicolumn{6}{c}{\textbf{RoBERTa}} & \multicolumn{6}{c}{\textbf{ElectraGen}} & \multicolumn{6}{c}{\textbf{Albert}} \\ 
    &  & cos & m-s & m-t & knn & svm & ffn & cos & m-s & m-t & knn & svm & ffn & cos & m-s & m-t & knn & svm & ffn & cos & m-s & m-t & knn & svm & ffn & cos & m-s & m-t & knn & svm & ffn \\ \midrule
    
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}} 
    & bathroom & 0.57* & 0.13 & 0.52* & 0.72* & 0.87* & 0.93* & 0.65* & 0.30 & 0.59* & 0.78* & 0.93* & 0.93* & 0.21 & 0.24 & 0.52* & 0.55* & 0.83* & 0.88* & 0.58* & 0.32 & 0.34 & 0.49* & 0.72* & 0.73* & 0.24 & 0.18 & 0.39 & 0.52* & 0.75* & 0.90* \\
    
    & bedroom & 0.48* & 0.33 & 0.43* & 0.53* & 0.66* & 0.77* & 0.44* & 0.41* & 0.44* & 0.44* & 0.87* & 0.78* & 0.23 & 0.18 & 0.36 & 0.17 & 0.53* & 0.60* & 0.32 & 0.31 & 0.37 & 0.37 & 0.37 & 0.39* & 0.23 & 0.22 & 0.47* & 0.31 & 0.44* & 0.68* \\
    
    & kitchen & 0.56* & 0.25 & 0.58* & 0.62* & 0.81* & 0.83* & 0.43* & 0.24 & 0.54* & 0.72* & 0.77* & 0.79* & 0.39 & 0.27 & 0.59* & 0.16 & 0.62* & 0.73* & 0.34 & 0.24 & 0.36 & 0.48* & 0.34 & 0.39* & 0.25 & 0.17 & 0.30 & 0.05 & 0.56* & 0.69* \\
    
    & living room & 0.30 & 0.37 & 0.26 & 0.51* & 0.78* & 0.79* & 0.23 & 0.38 & 0.24 & 0.57* & 0.49* & 0.66* & 0.13 & 0.38 & 0.28 & 0.49* & 0.74* & 0.65* & 0.26 & 0.48* & 0.33 & 0.15 & 0.27 & 0.26 & 0.15 & 0.35 & 0.54* & 0.20 & 0.29 & 0.40* \\
    
    & office & 0.46* & 0.39* & 0.28 & 0.40* & 0.59* & 0.61* & 0.40* & 0.37 & 0.31 & 0.25 & 0.52* & 0.71* & 0.14 & 0.37* & 0.38 & 0.18 & 0.74* & 0.63* & 0.17 & 0.37* & 0.23 & 0.42 & 0.27 & 0.36 & 0.23 & 0.22 & 0.42* & 0.45* & 0.66* & 0.81* \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.43* & 0.26* & 0.33* & 0.54* & 0.73* & 0.78* & 0.34* & 0.26* & 0.36* & 0.55* & 0.72* & 0.78* & 0.19* & 0.22* & 0.31* & 0.28* & 0.69* & 0.71* & 0.22* & 0.30* & 0.27* & 0.38* & 0.40* & 0.43* & 0.19* & 0.15 & 0.23* & 0.25* & 0.53* & 0.69* \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}} 
    & bed & 0.55* & 0.41* & 0.51* & 0.51* & 0.69* & 0.79* & 0.49* & 0.41* & 0.55* & 0.56* & 0.69* & 0.69* & 0.20 & 0.42* & 0.62* & 0.49* & 0.52* & 0.60* & 0.37* & 0.31* & 0.43* & 0.44* & 0.44* & 0.43* & 0.26 & 0.40* & 0.54* & 0.36* & 0.66* & 0.71* \\
    
    & dishwasher & 0.22 & 0.16 & 0.22 & 0.27 & 0.31* & 0.28* & 0.30* & 0.18 & 0.31* & 0.29* & 0.17 & 0.18 & 0.16 & 0.19 & 0.19 & 0.13 & 0.24 & 0.17 & 0.26 & 0.19 & 0.21 & 0.01 & 0.23 & 0.36* & 0.17 & 0.18 & 0.25 & 0.26 & 0.25 & 0.23 \\
    
    & door & 0.19 & 0.32* & 0.20 & 0.34* & 0.65* & 0.63* & 0.13 & 0.28 & 0.39* & 0.47* & 0.60* & 0.62* & 0.15 & 0.33* & 0.27 & 0.52* & 0.42* & 0.51* & 0.14 & 0.20 & 0.17 & 0.41* & 0.57* & 0.60* & 0.13 & 0.29* & 0.21 & 0.36* & 0.50* & 0.54* \\
    
    & mortise lock & 0.12 & 0.14 & 0.09 & 0.16 & 0.26 & 0.28* & 0.14 & 0.23 & 0.11 & 0.19 & 0.26 & 0.35* & 0.07 & 0.29* & 0.12 & 0.08 & 0.18 & 0.28 & 0.16 & 0.18 & 0.15 & 0.39 & 0.59* & 0.39* & 0.09 & 0.27* & 0.22 & 0.16 & 0.31* & 0.39* \\
    
    & refrigerator & 0.44* & 0.21 & 0.40* & 0.48* & 0.47* & 0.54* & 0.38* & 0.21 & 0.54* & 0.42* & 0.51* & 0.50* & 0.18 & 0.38* & 0.45* & 0.49* & 0.43* & 0.49* & 0.37* & 0.33* & 0.43* & 0.46* & 0.45* & 0.53* & 0.44* & 0.27* & 0.51* & 0.66* & 0.51* & 0.61* \\
    
    & toilet & 0.18 & 0.16 & 0.29* & 0.16 & 0.34* & 0.45* & 0.25 & 0.16 & 0.26 & 0.36* & 0.55* & 0.50* & 0.22 & 0.34* & 0.41* & 0.45* & 0.51* & 0.51* & 0.34* & 0.26 & 0.42* & 0.26 & 0.41* & 0.46* & 0.24 & 0.23 & 0.25 & 0.22 & 0.31* & 0.46* \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.20* & 0.20* & 0.24* & 0.33* & 0.45* & 0.49* & 0.22* & 0.21* & 0.28* & 0.39* & 0.46* & 0.46* & 0.07 & 0.29* & 0.29* & 0.39* & 0.39* & 0.43* & 0.21* & 0.19* & 0.23* & 0.32* & 0.45* & 0.47* & 0.08 & 0.23* & 0.27* & 0.35* & 0.42* & 0.49* \\ \midrule
    
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}} 
    & eat & 0.78* & 0.65* & 0.67* & 0.89* & 0.84* & 0.90* & 0.65* & 0.58* & 0.72* & 0.80* & 0.89* & 0.90* & 0.26 & 0.66* & 0.81* & 0.65* & 0.87* & 0.86* & 0.62* & 0.64* & 0.76* & 0.74* & 0.79* & 0.79* & 0.53* & 0.61* & 0.74* & 0.57* & 0.84* & 0.85* \\
    
    & listen to & 0.46* & 0.53* & 0.51* & 0.42* & 0.52* & 0.57* & 0.50* & 0.52* & 0.50* & 0.43* & 0.55* & 0.52* & 0.30 & 0.53* & 0.55* & 0.23 & 0.49* & 0.54* & 0.57* & 0.47* & 0.59* & 0.00* & 0.36* & 0.39* & 0.23 & 0.47* & 0.51* & 0.07 & 0.44* & 0.57* \\
    
    & play & 0.63* & 0.58* & 0.69* & 0.54* & 0.58* & 0.61* & 0.55* & 0.60* & 0.73* & 0.54* & 0.64* & 0.66* & 0.37 & 0.64* & 0.65* & 0.38* & 0.53* & 0.59* & 0.64* & 0.53* & 0.69* & 0.64* & 0.64* & 0.65* & 0.37 & 0.42* & 0.52* & 0.45 & 0.60* & 0.62* \\
    
    & read & 0.42* & 0.46* & 0.65* & 0.34 & 0.73* & 0.65* & 0.30 & 0.42* & 0.66* & 0.42* & 0.77* & 0.59* & 0.26 & 0.29 & 0.59* & 0.21 & 0.44* & 0.44* & 0.41* & 0.43* & 0.63* & 0.51* & 0.68* & 0.69* & 0.31 & 0.19 & 0.57* & 0.35 & 0.63* & 0.60* \\
    
    & wash with & 0.49* & 0.46* & 0.33* & 0.49* & 0.66* & 0.63* & 0.42* & 0.53* & 0.45* & 0.61* & 0.62* & 0.60* & 0.30 & 0.56* & 0.30 & 0.23 & 0.60* & 0.59* & 0.42* & 0.50* & 0.35* & 0.52* & 0.40 & 0.41 & 0.33 & 0.42* & 0.32 & 0.18 & 0.46* & 0.51* \\

    & wear & 0.66* & 0.64* & 0.76* & 0.88* & 0.90* & 0.92* & 0.62* & 0.57* & 0.74* & 0.79* & 0.90* & 0.85* & 0.24 & 0.64* & 0.77* & 0.36* & 0.72* & 0.79* & 0.53* & 0.62* & 0.74* & 0.90* & 0.84* & 0.83* & 0.30 & 0.61* & 0.77* & 0.61* & 0.77* & 0.86*  \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.53* & 0.53* & 0.38* & 0.59* & 0.69* & 0.71* & 0.37* & 0.50* & 0.44* & 0.60* & 0.73* & 0.68* & 0.20* & 0.55* & 0.37* & 0.28* & 0.59* & 0.64* & 0.49* & 0.51* & 0.37* & 0.60* & 0.61* & 0.62* & 0.15* & 0.40* & 0.26* & 0.29* & 0.62* & 0.67* \\
    
    \bottomrule
    \end{tabularx}
    \caption{All results of the contextual masked-language models. cos: Cosine Measure, m-s: Masked-Source Log Score, m-t: Masked-Target Log Score, knn: K-Nearest Neighbors, svm: Support Vector Machine, fnn: Feed-Forward Network.\T{(* indicates significant at p < 0.01)}}
    \label{tab:masked-score-summary}
\end{table*}


\begin{table*}
    \centering
    \setlength{\tabcolsep}{2pt}
    \tiny
    \begin{tabularx}{\linewidth}{+l ^l | ^X ^X ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X ^X ^X | ^X ^X ^X ^X ^X ^X ^X ^X }
    \toprule
    &  & \multicolumn{8}{c}{\textbf{GPT2}} & \multicolumn{8}{c}{\textbf{GPT-Neo}} & \multicolumn{8}{c}{\textbf{GPT-J}} \\ 
    &  & cos & p-s & p-s-l & p-t & p-t-l & knn & svm & ffn & cos & p-s & p-s-l & p-t & p-t-l & knn & svm & ffn & cos & p-s & p-s-l & p-t & p-t-l & knn & svm & ffn  \\ \midrule
    
    \multirow{5}{*}{\textbf{\rotatebox[origin=c]{90}{Room}}}
    & bathroom & 0.52* & 0.20 & 0.38* & 0.50* & 0.37* & 0.31 & 0.95* & 0.95* & 0.30 & 0.22 & 0.51* & 0.36 & 0.25 & 0.53* & 0.89* & 0.91* & 0.50* & 0.26 & 0.60* & 0.66* & 0.48* & 0.35 & 0.89* & 0.92* \\
    
    & bedroom & 0.26 & 0.31 & 0.23 & 0.47* & 0.38* & 0.26 & 0.61* & 0.54* & 0.19 & 0.33 & 0.21 & 0.53* & 0.48* & 0.55* & 0.49* & 0.57* & 0.24 & 0.32 & 0.23 & 0.62* & 0.48* & 0.33 & 0.70* & 0.64* \\
    
    & kitchen & 0.34 & 0.41* & 0.45* & 0.69* & 0.60* & 0.53* & 0.82* & 0.83* & 0.31 & 0.49* & 0.67* & 0.70* & 0.57* & 0.38* & 0.51* & 0.81* & 0.33 & 0.36* & 0.52* & 0.83* & 0.70* & 0.70* & 0.82* & 0.83* \\
    
    & living room & 0.21 & 0.43* & 0.26 & 0.41* & 0.33 & 0.16 & 0.27 & 0.46* & 0.26 & 0.57* & 0.39 & 0.60* & 0.44* & 0.28 & 0.13 & 0.48* & 0.21 & 0.50* & 0.47* & 0.67* & 0.45* & 0.46 & 0.40* & 0.63* \\
    
    & office & 0.13 & 0.21 & 0.43* & 0.37 & 0.23 & 0.31 & 0.44* & 0.73* & 0.33 & 0.30 & 0.43* & 0.46* & 0.34 & 0.24 & 0.53* & 0.72* & 0.23 & 0.36 & 0.53* & 0.49* & 0.39 & 0.37* & 0.52* & 0.69* \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.26* & 0.23* & 0.30* & 0.46* & 0.35* & 0.30* & 0.61* & 0.72* & 0.15 & 0.34* & 0.44* & 0.44* & 0.35* & 0.40* & 0.52* & 0.71* & 0.23* & 0.32* & 0.42* & 0.56* & 0.41* & 0.42* & 0.66* & 0.74* \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Part}}}
    & bed & 0.36* & 0.30 & 0.51* & 0.67* & 0.45* & 0.55* & 0.59* & 0.70* & 0.32* & 0.38* & 0.46* & 0.77* & 0.70* & 0.66* & 0.78* & 0.88* & 0.46* & 0.38* & 0.36* & 0.81* & 0.68* & 0.71* & 0.83* & 0.84* \\
    
    & dishwasher & 0.11 & 0.34* & 0.22 & 0.25 & 0.23 & 0.18 & 0.21 & 0.28* & 0.06 & 0.23 & 0.30* & 0.30* & 0.29* & 0.15 & 0.15 & 0.24 & 0.09 & 0.26 & 0.30* & 0.44* & 0.38* & 0.12 & 0.15 & 0.32* \\
    
    & door & 0.23 & 0.07 & 0.14 & 0.20 & 0.28 & 0.20 & 0.65* & 0.66* & 0.27 & 0.10 & 0.17 & 0.35* & 0.42* & 0.20 & 0.44* & 0.66* & 0.15 & 0.13 & 0.12 & 0.37* & 0.41* & 0.25 & 0.67* & 0.77* \\
    
    & mortise lock & 0.07 & 0.34* & 0.43* & 0.17 & 0.18 & 0.27 & 0.63* & 0.65* & 0.11 & 0.49* & 0.42* & 0.30 & 0.22 & 0.27 & 0.49* & 0.61* & 0.15 & 0.43* & 0.43* & 0.47* & 0.31* & 0.04 & 0.63* & 0.66* \\
    
    & refrigerator & 0.42* & 0.41* & 0.24 & 0.53* & 0.52* & 0.47* & 0.39* & 0.51* & 0.29* & 0.33* & 0.33* & 0.47* & 0.55* & 0.44* & 0.47* & 0.57* & 0.46* & 0.51* & 0.41* & 0.57* & 0.63* & 0.55* & 0.53* & 0.63* \\
    
    & toilet & 0.29* & 0.36* & 0.44* & 0.20 & 0.17 & 0.16 & 0.49* & 0.54* & 0.27 & 0.42* & 0.50* & 0.25 & 0.26 & 0.23 & 0.50* & 0.58* & 0.32* & 0.45* & 0.48* & 0.32* & 0.37* & 0.26 & 0.53* & 0.62* \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.14* & 0.24* & 0.28* & 0.28* & 0.25* & 0.29* & 0.47* & 0.54* & 0.12 & 0.30* & 0.34* & 0.37* & 0.36* & 0.32* & 0.46* & 0.57* & 0.16* & 0.34* & 0.32* & 0.42* & 0.43* & 0.33* & 0.54* & 0.62* \\ \midrule
    
    \multirow{6}{*}{\textbf{\rotatebox[origin=c]{90}{Verb}}}
    & eat & 0.49* & 0.82* & 0.65* & - & - & 0.82* & 0.87* & 0.87* & 0.45* & 0.86* & 0.66* & - & - & 0.76* & 0.87* & 0.88* & 0.48* & 0.68* & 0.74* & - & - & 0.63* & 0.89* & 0.89* \\
    
    & listen to & 0.22 & 0.57* & 0.51* & - & - & 0.29 & 0.50* & 0.58* & 0.22 & 0.47 & 0.47* & - & - & 0.20 & 0.42* & 0.55* & 0.21 & 0.60* & 0.56* & - & - & 0.29 & 0.52* & 0.60* \\
    
    & play & 0.40* & 0.64* & 0.62* & - & - & 0.62* & 0.61* & 0.59* & 0.32 & 0.66* & 0.61* & - & - & 0.20 & 0.55* & 0.62* & 0.34 & 0.66* & 0.70* & - & - & 0.37 & 0.67* & 0.67* \\
    
    & read & 0.32 & 0.63* & 0.30 & - & - & 0.32* & 0.45* & 0.45* & 0.32 & 0.61* & 0.34 & - & - & 0.29 & 0.52* & 0.49* & 0.40* & 0.63* & 0.41* & - & - & 0.20 & 0.59* & 0.49* \\
    
    & Wash with & 0.39* & 0.77* & 0.51* & - & - & 0.57* & 0.61* & 0.63* & 0.28 & 0.66* & 0.52* & - & - & 0.39 & 0.41 & 0.60* & 0.23 & 0.69* & 0.52* & - & - & 0.66* & 0.61* & 0.64* \\
    
    & wear & 0.44* & 0.38 & 0.72* & - & - & 0.76* & 0.84* & 0.87* & 0.16 & 0.39 & 0.66* & - & - & 0.68* & 0.79* & 0.85* & 0.21 & 0.38 & 0.62* & - & - & 0.87* & 0.84* & 0.87* \\ \hline
    
    \rowstyle{\bfseries} & CONC & 0.31* & 0.52* & 0.53* & - & - & 0.51* & 0.64* & 0.66* & 0.19* & 0.49* & 0.52* & - & - & 0.40* & 0.59* & 0.66* & 0.23* & 0.50* & 0.56* & - & - & 0.48* & 0.68* & 0.69* \\

    \bottomrule
    \end{tabularx}
    \caption{All results of the contextual causal-language models. p-s: Predict Source Score, p-s-l: : Predict Source Log Score, p-t: Predict Target Score, p-t-l: Predict Target Log Score. The gap for the verb p-t score is due to the lack of an easily applicable sentence templates in this direction. \T{(* indicates significant at p < 0.01)}}
    \label{tab:gpt-score-summary}
\end{table*}
